A Better Resource Allocation Algorithm with Semi-Bandit Feedback

We study a sequential resource allocation problem between a fixed number of arms. On each iteration the algorithm distributes a resource among the arms in order to maximize the expected success rate. Allocating more of the resource to a given arm increases the probability that it succeeds, yet with a cut-off. We follow Lattimore et al. (2014) and assume that the probability increases linearly until it equals one, after which allocating more of the resource is wasteful. These cut-off values are fixed and unknown to the learner. We present an algorithm for this problem and prove a regret upper bound of $O(\log n)$ improving over the best known bound of $O(\log^2 n)$. Lower bounds we prove show that our upper bound is tight. Simulations demonstrate the superiority of our algorithm.

==> multi-exclusive.tex <==

\section{Multi-armed exclusive problem} 
\yd{this is a natural generalization of the one armed algorithm, which
	I could add with no much effort.
	I think it contributes to the understanding.
	Mainly because it is defined similarly as the regular multi armed bandit,
	but its regret can be much lower. 
	If there is no room, or if we think that it takes too much attention from the main problem,
	we can remind it just briefly in a subsection of the single armed bandit problem, or in one paragraph + theorem.}

Assume that there are $\nban$ arms, with parameters $0 < \amt_1, \dots, \amt_{\nban} \le 1$,
each with the same behavior as in the one-arm problem.
Let $\amt^* = \min_{1\le k \le \nban} \amt_k$ be the minimum of these values. 
The algorithm does not know which arm is $\amt_1$.
There are $n$ rounds, and in every round $1 \le t \le n$ the algorithm grants $\alloc_t$ resources to one of the arms,
invokes it, and observes its success status $\scc_t$.
The algorithm is then compared to the optimal allocation that knows which arm has the smallest demand,
and allocates resources only to this arm for $n$ rounds.
The goals are as in the one arm problem, namely:
\begin{enumerate}
	\item
		Minimize $\sum_{t=1}^n (\alloc_t - \amt^*)$, the amount of resource allocated by the algorithm,
		minus the amount required in order to guarantee no failure.
	\item
		Minimize $\sum_{t=1}^n (1 - \scc_t)$, the number of failures.
\end{enumerate}

We suggest an algorithm, which is a simple generalization of Algorithm~\ref{alg:one-arm}, the one-arm algorithm.
It maintains the states of $\nban$ instances of Algorithm~\ref{alg:one-arm}, one for each arm.
The algorithm gets a parameter $\mulc$ as an inputs, and invokes each of the $\nban$ instances of with this value of $\mulc$ as an input.
The lower bound for arm $k$ calculated on iteration $t$ is denoted $\lb_{k,t}$.
In every iteration the arm with the lowest lower bound value is invoked.
The pseudo-code appears under the name Algorithm~\ref{alg:om}.

\begin{algorithm} 
	\caption{Multi armed - single allocated each time \cmt{rename}} 
	\begin{algorithmic}[1] \label{alg:om}
		\STATE$\lb_{k,0} \gets 0$ for all $1 \le k \le \nban$ 
		\FORALL {$t \in \{1, 2, \dots\}$}
		\STATE $k_t \gets \arg\min_{1 \le k \le \nban} \lb_{k,t-1}$.
		\STATE $n_t \gets$ the number of times arm $k_t$ was invoked on iterations $1, \dots, t-1$
		\STATE $\alloc_t \gets \lb_{k_t, t-1} + \frac{\mulc}{n_t+1}$
		\STATE Grant the arm $k_t$ with $\alloc_t$ resources
		\STATE $\scc_t \gets$ success status of the arm
		\IF{$\scc_t = 1$}
		\STATE $\lb_{k_t,t} \gets \lb_{t-1}$
		\ELSE
		\STATE $\lb_{k_t,t} \gets \alloc_t$
		\ENDIF
		\STATE $\lb_{k,t} \gets \lb_{k,t-1}$ for all $k \ne k_t$
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

The guarantees are similar to those in the one-arm problem:
if there is a unique minimizer for $\amt_1, \dots, \amt_\nban$,
both the amount of excess allocated resource, and the number of failures,
are bounded by $O(\log n)$, plus some term which is independent of $n$.
The constant multiplying the $\log n$ term is independent of $\nban$.
This is better than the optimal regret achievable in a standard stochastic multi armed bandit
problem (\cite{LR}), where the regret is $\Omega(\nban \log n)$ in general.
Furthermore, these two guarantees of the algorithm have a logarithmic upper bound,
which is independent of the parameters $\amt_1, \dots, \amt_\nban$:
for any $n$, and any $\nban$ armed problem,
the excess resource allocation is bounded by $\mulc \nban \log n$,
and the expected number of failures by $\frac{\mulc}{\mulc-1} \nban \log n$.
The worst problems for this algorithm are those where
$\amt_1 = \amt_2 = \cdots = \amt_\nban$.
This is in contrast to the standard multi armed setting, where for any value of $n$
there are hard instances with $\nban = 2$ arms, with a lower bound of
$\Omega\left( \sqrt{n} \right)$ on the regret.
\cmt{add a citation}
The following theorem formally states the guarantees of the algorithm.

\begin{theorem} \label{thm:om}
	Fix $0 < \amt_1, \amt_2, \dots, \amt_\nban \le 1$,
	and let $\amt^* = \min(\amt_1, \dots, \amt_\nban)$.
	Assume that Algorithm~\ref{alg:om} is invoked with parameter $\mulc > 1$
	on these arms, for $n$ iterations.
	
	Then, the following guarantees hold:
	\begin{enumerate}
		\item \label{itm:th-om-1}
		$\E \left[ \sum_{t=1}^n (\alloc_t - \amt^*) \right] 
		\le \sum_{k=1}^\nban \min\left( c \log n, C \log \frac{1}{\amt_k - \amt^*} + C \right)$
		\item \label{itm:th-om-2}
		$\E \left[ \sum_{t=1}^n (1 - \scc_t) \right] 
		\le \sum_{k=1}^\nban \min\left( \frac{c}{c-1} \log n, C \log \frac{1}{\amt_k - \amt^*} + C \right)$
	\end{enumerate}
	where $\log \frac{1}{0}= \infty$, and
	$C > 0$ is some constant which depends only on $\mulc$.
\end{theorem}

\subsection{Proof of Theorem~\ref{thm:om}}
Fix an arm $1 \le k \le \nban$.
Let $n'$ be the number of times that arm $k$ is invoked throughout the $n$ iterations of the algorithm,
and let $t_1 < \cdots < t_{n'}$ be these iterations.
We start by proving item~\ref{itm:th-om-1}.
It is sufficient to prove that 
\begin{equation} \label{eq:omm-0}
	\E \left[ \sum_{i=1}^{n'} (\alloc_{t_i} - \amt^*) \right] 
	\le \min\left( c \log n, C \log \frac{1}{\amt_k - \amt^*} + C \right).
\end{equation}

The guarantee for the one-arm problem, proved in Theorem~\ref{thm:ub-one},
states that the left hand side of \eqref{eq:omm-0} is bounded by $c \log n$.
Next, we prove that it is bounded by $C \log \frac{1}{\amt_k - \amt^*}$, whenever $\amt_k > \amt^*$, to complete the proof of \eqref{eq:omm-0}.

Assume therefore that $\amt_k > \amt^*$.
Next, we show that for all $1 \le i \le n'$,
\begin{equation} \label{eq:omm-3}
	\lb_{k,t_i-1} < \amt^*.
\end{equation}
Since arm $k$ is invoked by the algorithm on iteration $t_i$, it has the minimal lower bound on this iteration, namely,
$\lb_{k,t_i-1} = \min_{1\le s \le \nban} \lb_{s,t_i-1}$.
Let $s$ be the arm which satisfies $\amt_s = \amt^*$.
It holds that $\lb_{k,t_i - 1} \le \lb_{s,t_i - 1} < \amt_s = \amt^*$, which completes the proof of \eqref{eq:omm-3}.

Let $n_1 = \min \para{n', \left\lceil \frac{2 \mulc}{\amt - \amt^*}\right\rceil - 1}$.
We will split the left hand side of \eqref{eq:omm-0} to two sums, one from $1$ to $n_1$,
and the other from $n_1+1$ to $n'$.
The first sum is bounded by
\begin{align}
	\sum_{i=1}^{n_1} (\alloc_{t_i} - \amt^*)
	&= \sum_{i=1}^{n_1} \left(\lb_{k,t_i - 1} + \frac{\mulc}{i} - \amt^* \right) \nonumber\\
	&\le \sum_{i=1}^{n_1} \frac{\mulc}{i} \label{eq:omm2} \\
	& \le \mulc \para{ \log n_1 + 1} \nonumber \\
	& \le \mulc \para{ \log \frac{2 \mulc}{\amt - \amt^*} + 1} \nonumber.
\end{align}
where \eqref{eq:omm2} follows from \eqref{eq:omm-3}.

Proceed with bounding the sum from $n_1+1$ to $n'$.
If $n' = n_1$ it trivially equals zero, therefore assume that $n' > n_1$.
For any $n_1 < i \le n'$ it holds that
\begin{equation} \label{eq:omm4}
	\alloc_{t_i}
	= \lb_{k,t_i-1} + \frac{\mulc}{i}
	\le \amt^* + \frac{\mulc}{n_1+1}
	\le \amt^* + \frac{\amt_k - \amt^*}{2}.
\end{equation}
where the second step follows from \eqref{eq:omm-3}.

Let $i_1 < \cdots < i_m$ denote all values of $n_1 < i \le n'$, for which $\alloc_{t_i} > \amt^*$.
It holds that
\begin{align}
	\sum_{i=n_1+1}^{n'} (\alloc_{t_i} - \amt^*)
	&\le \sum_{j=1}^{m} (\alloc_{t_{i_j}} - \amt^*) \nonumber\\
	&\le \sum_{j=1}^{m} \frac{\amt_k - \amt^*}{2} \label{eq:omm5} \\
	&= m \frac{\amt_k - \amt^*}{2} \nonumber,
\end{align}
where \eqref{eq:omm5} follows from \eqref{eq:omm4}.
We will show that $\E m \le \frac{2}{\amt_k - \amt^*}$,
thereby, completing the proof of \eqref{eq:omm-0}.

First, note that for any $j < m$ it holds that
the arm succeeds on iteration $t_{i_j}$, namely, 
$\scc_{t_{i_j}} = 1$.
Otherwise, it would hold that
\[
\lb_{k, t_{i_{j+1}}}
\ge \lb_{k, t_{i_{j}}}
= \alloc_{k, t_{i_{j}}}
> \amt_k,
\]
where the first and second steps follow from the definition of the algorithm,
and the last step follows from the definition of $j_1, \dots, j_m$.
This contradicts \eqref{eq:omm-3}, and proves that $\scc_{t_{i_j}} = 1$ 
for all $j < m$ as required.

For any $1 \le j \le m$, \eqref{eq:omm4} implies that
$\amt_k - \alloc_{t_{i_j}} \ge \frac{\amt_k - \amt^*}{2}$.
The definition of the problem implies that the probability that the arm fails on iteration $t_{i_j}$, and $\scc_{t_{i_j}} = 0$,
is at least $\amt_k - \alloc_{t_{i_j}} \ge \frac{\amt_k - \amt^*}{2}$.
Viewing $m$ as a random variable, this implies that for any integer $j > 0$, 
\[
\Pr[m \ge j + 1 \mid m \ge j]
\le \Pr\left[\alloc_{t_{i_j}} = 1 \mid m \ge j \right]
\le 1 - \frac{\amt_k - \amt^*}{2}.
\]
Therefore, $m$ can be bounded by a geometric random variable with parameter $\frac{\amt_k - \amt^*}{2}$,
which implies that $\E m \le \frac{2}{\amt_k - \amt^*}$ as required. This completes the proof of \eqref{eq:omm-0},
and item~\ref{itm:th-om-1} of the theorem follows.

Next, we prove the second part of the theorem.
It is sufficient to prove that
\begin{equation} \label{eq:omm2-m}
	\E \left[ \sum_{i=1}^{n'} (1 - \scc_{t_i}) \right] 
	\le \min\left( \frac{\mulc}{\mulc-1} \log n, C \log \frac{1}{\amt_k - \amt^*} + C \right).
\end{equation}
Using Theorem~\ref{thm:ub-one} for the one-arm problem,
it holds that 
\[
\E \left[ \sum_{i=1}^{n'} (1 - \scc_{t_i}) \right] 
\le \frac{\mulc}{\mulc-1} \log n.
\]
Next, we will bound this quantity by $C \log \frac{1}{\amt_k - \amt^*} + C$
assuming that $\amt_k > \amt^*$, and it suffices to complete the proof.
Inequality~\eqref{eq:omm-3} implies that it suffices to bound the number of failures of arm $k$
before the first iteration $t$ when $\lb_{k,t} \ge \amt^*$.
This implies that the following lemma suffices to complete the proof.

\begin{lemma}
	Fix some $0 < a < \amt \le 1$.
	Assume that the one armed algorithm, Algorithm~\ref{alg:one-arm}, runs and interacts with an arm with parameter $\amt$,
	and gets an input parameter $\mulc > 1$.
	Let $\alloc_t$, $\scc_t$ and $\lb_t$ be defined as in the algorithm for all $t = 1,2,\cdots$.
	Let $\rvt$ be the first iteration $t$ such that $\lb_t > a$.
	Then,
	\[ \E\left[ \sum_{t=1}^{\rvt} (1 - \scc_t) \right] \le C\log \frac{1}{\amt - a} + C, \]
	where $C > 0$ is some parameter which depends only on $\mulc$.
\end{lemma}

\begin{proof}
	We will prove that for any iteration $t \ge 1$, and any value $0 \le \lb_{t-1} < \amt$,
	\begin{equation} \label{eq:om-main}
		\E \left[ \sum_{i=t}^{\rvt} (1 - \scc_i) \middle\vert t, \lb_{t-1} \right]
		\le \phi(\amt - \lb_{t-1}, t),
	\end{equation}
	where
	\[
	\phi(\err,t) = c_1 \left( \log \frac{2 \err}{\amt - a} \right)_+ + c_2 (\err t - \alpha)_+,
	\]
	where the function $(\cdot)_+$ denotes $\max(0, \cdot)$, and 
	\begin{align*}
		\gamma_1 &= \frac{2 \mulc^2}{\mulc - 1} \\
		\alpha &= \gamma_1 + 1 \\
		\gamma_2 &= \alpha + \mulc \\
		c_2 &= \frac{2}{\mulc-1} \\
		c_1 &= \frac{2 c_2 + 1}{\log \frac{1}{1 - \mulc / \gamma_2}}.
	\end{align*}
	Whenever $\amt - \lb_{t-1} < \amt - a$, the left hand side of inequality~\eqref{eq:om-main} is trivially zero,
	and the right hand side is always nonnegative, therefore \eqref{eq:om-main} holds.
	Therefore, for the next of the proof we assume thats $\amt - \lb_{t-1} < \amt - a$.
	
	Fix some values of $t$ and $\lb_{t-1}$.
	Denote $\err = \amt - \lb_{t-1}$. Denote $t_0 = t_1 = t$.
	Denote by $\err_0$ the value $\amt - \lb_t$ gets if $\scc_t = 0$, namely, $\err_0 = (\err - \frac{\mulc}{t})_+$.
	Similarly, let $\err_1$ be the value of $\amt - \lb_t$ if $\scc_t = 1$, namely, $\err_1 = \err$.
	Let $p$ be the probability that $\scc_t$ equals $0$, given $\lb_{t-1}$.
	In order to prove \eqref{eq:om-main}, it is sufficient to prove the following inductive inequality:
	\begin{equation} \label{eq:om-rec}
		\phi(\err, t) \ge p \left( \phi(\err_0, t_0) + 1 \right) + (1-p) \phi(\err_1, t_1) .
	\end{equation}
	
	The proof of \eqref{eq:om-rec} will be divided into cases.
	First, it assumes that $\err_ 0 \ge \frac{\amt - a}{2}$,
	and proves for each of the following three cases:
	$t \err < \gamma_1$, $\gamma_1 \le t \err \le \gamma_2$,
	and $t \err > \gamma_2$.
	Lastly, it proves for the case that $\err_ 0 \ge \frac{\amt - a}{2}$.
	
	Start by assuming that $\err_ 0 \ge \frac{\amt - a}{2}$.
	It holds that, $\log \frac{2 \err_0}{\amt - a} \ge 0$, therefore
	\begin{equation} \label{eq:om-e0-good}
		\left( \log \frac{2 \err_0}{\amt - a} \right)_+
		= \log \frac{2 \err_0}{\amt - a}.
	\end{equation}
	
	It holds that if $t \err \le \gamma_2$,
	then 
	\begin{equation} \label{eq:om-0}
		c_1 \log \frac{\err}{\err_0} - 1 
		= c_1 \log \frac{\err}{\err - \mulc/t} - 1 
		= c_1 \log \frac{1}{1 - \mulc/(\err t)} - 1 
		\ge c_1 \log \frac{1}{1 - \mulc/\gamma_2} - 1 
		= 2 c_2.
	\end{equation}
	
	If $t \err \ge \gamma_1$, then
	\begin{equation} \label{eq:om-1}
		\err_0
		= \err - \frac{\mulc}{t}
		= \err \left( 1 - \frac{\mulc}{\err t} \right)
		\ge \err \left( 1 - \frac{\mulc}{\gamma_1} \right)
		= \err \left( 1 - \frac{\mulc(\mulc - 1)}{2 \mulc^2} \right)
		\ge \err / 2.
	\end{equation}
	Therefore, if $t \err \ge \gamma_1$ then 
	\begin{equation} \label{eq:om-2}
		p = \err - \frac{\mulc}{t} \ge \err / 2.
	\end{equation}
	
	Therefore, if $\gamma_1 \le t \err \le \gamma_2$, then
	\begin{align}
		&\phi(\err, t) - p \left( \phi(\err_0, t_0) + 1 \right) - (1-p) \phi(\err_1, t_1) \nonumber\\
		&= -p + p c_1 \log \frac{\err}{\err_0} + c_2 (\err t - \alpha)_+ 
		- p c_2(\err_0(t+1) - \alpha)_+ - (1-p) c_2(\err_1(t+1) - \alpha)_+ \label{eq:om-3} \\
		&\ge -p + p c_1 \log \frac{\err}{\err_0} + c_2 (\err t - \alpha)_+ - c_2(\err(t+1) - \alpha)_+ \nonumber\\
		&\ge p \left( c_1 \log \frac{\err}{\err_0} - 1 \right) - c_2 \err \nonumber \\
		&\ge \frac{2p}{c_2} - c_2 \err \label{eq:om-4} \\
		&\ge 0. \label{eq:om-5} \\
	\end{align}
	where \eqref{eq:om-3} follows from \eqref{eq:om-e0-good},
	\eqref{eq:om-4} follows from \eqref{eq:om-0},
	and \eqref{eq:om-5} follows from \eqref{eq:om-2}.
	This concludes the proof of \eqref{eq:om-rec} for the case that $\gamma_1 \le t \err \le \gamma_2$.
	
	Next, assume that $t \err > \gamma_2$. Then,
	\begin{equation} \label{eq:om-6}
		t \err_0
		= t \left( \err - \frac{\mulc}{t} \right)
		= t \err - \mulc.
	\end{equation}
	Therefore,
	\begin{equation} \label{eq:om-7}
		t \err
		\ge t \err_0
		\ge t \err - \mulc
		\ge \gamma_2 - \mulc
		= \alpha.
	\end{equation}
	Additionally,
	\begin{equation} \label{eq:om-10}
		\mulc p - \err
		= \mulc \left( \err - \frac{\mulc}{t} \right) - \err 
		= \err \left( \mulc - 1 - \frac{\mulc^2}{\err t} \right)
		\ge \err \left( \mulc - 1 - \frac{\mulc^2}{\gamma_2} \right)
		\ge \err \left( \mulc - 1 - \frac{\mulc^2}{\gamma_1} \right)
		= \frac{\mulc - 1}{2} \err.
	\end{equation}
	This concludes that,
	\begin{align}
		&\phi(\err, t) - p \left( \phi(\err_0, t_0) + 1 \right) - (1-p) \phi(\err_1, t_1) \nonumber \\
		&\ge -p + c_2 (\err t - \alpha)_+ - p c_2 (\err_0 (t+1) - \alpha)_+ - (1-p)c_2 (\err_1 (t+1) - \alpha)_+ \nonumber \\
		&= -p + c_2 \left( \err t - p \err_0 (t+1) - (1-p) \err (t+1) \right)\label{eq:om-8} \\
		&\ge -p + c_2 \left( p(\err t - \err_0 t) - \err \right) \nonumber \\
		&= -p + c_2 (\mulc p - \err) \label{eq:om-9} \\
		&\ge -p + c_2 \frac{\mulc - 1}{2} \err  \label{eq:om-11} \\
		&= -p + \err \nonumber \\
		&\ge 0 \nonumber.
	\end{align}
	where \eqref{eq:om-8} follows from \eqref{eq:om-7},
	\eqref{eq:om-9} follows from \eqref{eq:om-6},
	and \eqref{eq:om-11} follows from \eqref{eq:om-10}.
	This completes the proof for the case that $\err t > \gamma_2$.
	
	Next, assume that $\err t < \gamma_1$.
	This implies that
	\begin{equation} \label{eq:om-12}
		\err (t+1)  
		= \err t + \err
		\le \gamma_1 + 1
		= \alpha.
	\end{equation}
	Therefore,
	\begin{align}
		&\phi(\err, t) - p \left( \phi(\err_0, t_0) + 1 \right) - (1-p) \phi(\err_1, t_1) \nonumber \\
		&= p(c_1 \log \frac{\err}{\err_0} - 1) \label{eq:om-13} \\
		&\ge 2 p c_2 \label{eq:om-14} \\
		&\ge 0,
	\end{align}
	where \eqref{eq:om-13} follows from \eqref{eq:om-12} and \eqref{eq:om-e0-good},
	and \eqref{eq:om-14} follows from \eqref{eq:om-0}.
	This completes the proof of \eqref{eq:om-rec} for the case $\err t < \gamma_1$.
	
	Lastly, assume that $\err_0 < \frac{\amt-a}{2}$.
	It holds that
	\begin{equation*}
		\frac{c}{\gamma_2}
		\le \frac{c}{\gamma_1}
		= \frac{c(c-1)}{2 c^2}
		\le \frac{1}{2}.
	\end{equation*}
	Therefore, 
	\begin{equation} \label{eq:om-15}
		c_1
		\ge \log^{-1} \frac{1}{1-c/\gamma_2}
		\ge \log^{-1} 2.
	\end{equation}
	Additionally, since $\err_0 < \frac{\amt-a}{2}$, 
	it holds that $t \err < \gamma_1$, otherwise \eqref{eq:om-1} would imply that
	$\err_0 \ge \frac{\err}{2} \ge \frac{\amt-a}{2}$.
	Therefore, \eqref{eq:om-12} holds.
	For conclusion,
	\begin{align}
		&\phi(\err, t) - p \left( \phi(\err_0, t_0) + 1 \right) - (1-p) \phi(\err_1, t_1) \nonumber \\
		&= -p + p c_1 \log \frac{2\err}{\amt - a} \label{eq:om-16} \\
		&\ge -p + p c_1 \log 2 \nonumber \\
		&\ge 0 \label{eq:om-17}
	\end{align}
	where \eqref{eq:om-16} follows from \eqref{eq:om-12},
	and \eqref{eq:om-17} follows from \eqref{eq:om-15}.
	This completes the proof of \eqref{eq:om-rec},
	and the proof of the theorem follows.
\end{proof}



==> multi-outline.tex <==
\section{Proof Outline of Theorem~\ref{thm:multi-arm}} \label{sec:pr-outline}

%We start by presenting an outline of the proof, which contains the main
%idea and a summary of their proofs.
%The proofs of the lemmas, together with a list of all definitions appears in the appendix.
%This section contains many technical definitions,
%which are, for themselves, not very interesting,
%yet they are essential for understanding the proof and all lemmas are based on then.
%Since the algorithm does not know the number of iterations in advance, it is impossible
%to make adjustments to the algorithm that rely on this information.
%This complicates the proof and requires us to analyze the behavior of the algorithm for any state it gets to,
%which results in a highly technical proof.
%
%We bound the expected regret of the algorithm after $n$ rounds if it interacts with the fixed arms $\amt_1, \dots, \amt_\nban$.
%The algorithm gets as an input a parameter $\mulc$, which is used for calculating the value of $\add_{k,t}$.
%It is conseders as a constant ,and indeed, it can get any constant value higher than $2$,
%to the choice of the user.
%
%For convenience, for any iteration $1 \le t \le n$, let $\regret_t$ be the difference between the \emph{expected}
%reward of the optimal allocation, and the \emph{actual} reward by the algorithm, namely,
%\[
%	\regret_t = \nal + \indi_{\nban > \nal} \frac{\rem}{\amt_{\nal+1}} - \sum_{k=1}^\nban \scc_{k,t}.
%\]
%It holds that $\regret^{(n)} = \E \left[ \sum_{t=1}^n \regret_t \right]$.
%
%The algorithm maintains a lower bound $\lb_{k,t}$ for any arm $1 \le k \le \nban$ and iteration $1 \le t \le n$.
%Most of the proof relates only to iterations $t$ such that for any arm $k$, this lower bound is positive and less than $\amt_k$.
%Let $T$ be the set of these iterations, namely, 
%\[  T = \{ t \colon 1 \le t \le n,\ 0 < \lb_{k,t} \le \amt_k \text{ for all } 1 \le k \le \nban \}. \]
%For any iteration $t \notin T$, the regret $R_t$ is bounded trivially as if no reward is gained from these iterations, namely, we bound $R_t \le \nal + 1$.
%Later on this outline, we state a lemma that bounds the expected number of iterations not in $T$.
We now sketch a proof outline of \thmref{thm:multi-arm}. We start by
splitting the iterations into two types.  Let $T$ be the set of ``good
iterations'', for which $0 < \lb_{k,t-1} \le \amt_k$ for all $k$. The
core of the proof relates to iterations $t \in T$, while the number of
iterations $t \notin T$ can be bounded %mainly 
utilizing Azuma's
inequality to bound the number of iterations for which
$\lbs_{k,t} > \amt_k$.
\begin{lemma} \label{lem:notin-T}
	The expected number of iterations $t \notin T$ is bounded by
	$C \max\left(\log \frac{1}{\amt_1}, 1\right)$,
	for some constant $C > 0$, depending only on $\mulc$.
\end{lemma}
%
%We start by describing how the regret is bounded in ``good iterations'' when $t \in T$.
%The optimal allocation that knows the parameters $\amt_1, \dots, \amt_k$,
%allocates the first $\nal$ arms with the amount they require,
%and the next arm gets the remaining of the resource (this happens in case there is no sufficient resource for all arms.
%There are $\nal + 1$ arms which are allocated with a non-negative amount of resource.
%The regret in an iteration $t \in T$ is calculated by comparing the reward obtained by the ``optimal'' allocation,
%with the reward obtained by at most $\nal + 1$ arms in the algorithm.
%For this purpose, three sets of arms, $A_t$, $B_t$ and $C_t$, will be defined,
%and only the reward of the arms in these sets is going to be considered for the calculation of the regret.
%Optimally, the set $A_t$ would contain the $\nal$ arms that get the highest priority by the algorithm on iteration $t$,
%where the arm with the next priority is going to be located either in $B_t$ or $C_t$:
%one of these two sets is going to be a singleton which contains only this arm, and the other is going to be empty.
%In reality, however, $A_t$ is not necessarily going to contain exactly $\nal$ arms. It might be the case that $A_t$
%contains $\nal + 1$ arms, and when it happens $B_t$ and $C_t$ are both empty.
%Additionally, $A_t$ can be of size less than $\nal$.
%It holds that $A_t$, $B_t$ and $C_t$ are subsets of the sets of arms labeled by $A$, $B$ and $C$ by the algorithm on iteration $t$, respectively.

From now we focus on the iterations $t
\in T$ (i.e. the lower bound is indeed correct), and will bound the
the reward achieved by the algorithm only on arms 
in the sets $A_t$, $B_t$ and $C_t$ which are
subsets of the arms of cases A, B, and C (to be defined).

% is bounded considering only arms in
% the sets $A_t$, $B_t$ and $C_t$, which are subsets of the arms in cases A, B and C, respectively
% (to be defined).
Let $k_{1,t}, \dots, k_{\nban,t}$ be an ordering of the arms such that arm $k_i$
is located in the i$th$ position in the loop over the arms in line~\ref{algl:k-loop} of the algorithm,
ordering the arms ascending over $\lb_{k,t-1}$.
%From the definition of the algorithm it holds that this ordering sorts the bandits in an increasing order of their maximum lower bound $\lb_{k,t} = \max(\lbf_{k,t}, \lbs_{k,t})$, namely $\lb_{k_{1,t},t-1} \le \lb_{k_{2,t},t-1} \le \cdots \le \lb_{k_{\nban,t},t-1}$.
%
Let $\nal_t$ be the number of arms processed in this loop before 
encountering an arm $k$ for which the amount of resource left is less than 
$\lbf_{k,t-1} + \add_{k,t}$.
%Formally, $\nal_t$ is the highest value of $i$ such that for all 
%$1 \le j \le i$, $\alloc_{k_{j,t}, t} = \lbf_{k_{j,t},t-1} + \add_{k_{j,t},t}$.
%Let $A_t$ be the set that contains the first $\nal+1$ arms encountered in that loop before the first time that there was an arm which did not have sufficient resource, or, in other words, $A_t$ contains the first $\min(\nal_t, \nal + 1)$ arms encountered in the loop. 
Let $A_t$ be the set containing the first $\min(\nal_t, \nal + 1)$
arms, % encountered,
\(
	A_t = \{ k_{1,t}, k_{2,t}, \dots, k_{\min(\nal_t, \nal+1),t}
        \}. 
\)
If $A_t$ contains less than $\min(\nal + 1, \nban)$ arms,
let $k'_t$ be the next arm encountered in the loop,
$k'_t = k_{|A_t|+1,t}$,
%and it is defined only if $|A_t| < \min(\nban, \nal + 1)$.
and otherwise $k'_t$ is undefined.
The remaining resource for $k'_t$ on iteration $t$ are less than $\lbf_{k,t-1} + \add_{k,t}$,
otherwise it would have been placed in $A_t$.
The arm $k'_t$ is either placed in $B_t$ or in $C_t$, depending on whether $k'_t$
is of case B or C, and no other arm is placed in these two sets. Formally,
%if the remaining resource for $k'_t$ surpass the lower bound $\lbf_{k,t-1}$, then $B_t = \{ k'_t \}$ and $C_t = \emptyset$
%(the actual amount of resource given to $k'_t$ is not necessarily higher than $\lbf_{k,t-1}$. This is defined depending on the random coin flip performed by the algorithm).
%If the amount of resource remaining is not higher than the lower bound, we set $C_t = \{k'_t \}$ and $B_t = \emptyset$.
%If $k'_t$ is not defined at all, which happens whenever $A_t$ is
%sufficiently large, then $B_t = C_t = \emptyset$.
\begin{align*}
B_t = \{k'_t \} \textrm{~~if~~} |A_t| < \min(\nal + 1,\nban) \ \BR{AND}\
1 - \sum_{k \in A_t} \alloc_{k,t} > \lbf_{k'_t,t-1} \quad\quad\textrm{~and~~}
B_t =\emptyset\textrm{~otherwise}~.
\\
C_t = \{k'_t \} \textrm{~~if~~} |A_t| < \min(\nal + 1,\nban) \ \BR{AND}\
1 - \sum_{k \in A_t} \alloc_{k,t} \leq \lbf_{k'_t,t-1} \quad\quad\textrm{~and~~}
C_t =\emptyset\textrm{~otherwise}~.
\end{align*}
%
% \begin{align*}
% B_t &= \begin{cases}
% \{k'_t \} & |A_t| < \min(\nal + 1,\nban) \ \BR{AND}\  1 - \sum_{k \in A_t} \alloc_{k,t} > \lbf_{k'_t,t-1} \\
% \emptyset & \BR{otherwise}
% \end{cases}, \\
% C_t &= \begin{cases}
% \{k'_t \} & |A_t| < \min(\nal + 1,\nban) \ \BR{AND}\  1 - \sum_{k \in A_t} \alloc_{k,t} \le \lbf_{k'_t,t-1} \\
% \emptyset & \BR{otherwise}
% \end{cases}.
% \end{align*}
If $B_t \ne \emptyset$, define
by $\add'_t$ the difference between the amount of resource left for $k'_t$ and its lower bound $\lbf_{k'_t,t-1}$, a value which is always positive, and if $B_t = \emptyset$ we define $r'_t = 0$:
%From the definition of $B_t$, this value is guaranteed to be positive.
%If $B_t = \emptyset$ then this value has no meaning and is defined to be $0$.
%Formally,
\[
	\add'_t = 1 - \sum_{k \in A_t} \alloc_k - \lbf_{k'_t,t-1}
        \quad\textrm{~~if~~}  B_t \ne \emptyset \quad\quad\quad\textrm{and}\quad\quad
        \add'_t=0 \quad\textrm{~~if~~} B_t = \emptyset~.
\]
% \[
% 	\add'_t = \begin{cases}
% 		1 - \sum_{k \in A_t} \alloc_k - \lbf_{k'_t,t-1} & B_t \ne \emptyset \\
% 		0 & B_t = \emptyset
% 	\end{cases}.
% \]

%Define by $Z_t$ the random variable that contains everything the algorithm has seen up to and just before the point it gets to see the success statuses of the arms on iteration $t+1$. It contains all the success statuses $\scc_{k,i}$ for any arm $1 \le k \le \nban$ and any iteration $1 \le i \le t$, in addition to all the randomness of the algorithm up to and including iteration $t + 1$.
%Particularly, the amounts allocated to the arms on iteration $t+1$, namely, $\alloc_{1,t+1}, \dots, \alloc_{\nban, t+1}$, are deterministically defined given $Z_t$.
%The expected regret in iteration $t$ given $Z_{t-1}$ therefore equals the expected reward of the optimal algorithm, 
%minus the expected reward of Algorithm~\eqref{alg:multi-arm}, which equals
Define by $Z_t$ the random variable which contains all the history up to the point where all
$\alloc_{1,t+1}, \dots, \alloc_{\nban,t+1}$ are defined
(it contains the values $\{ \scc_{k,i} \}_{1\le k \le \nban,i\le t}$ and the randomness of the algorithm up to and including iteration $t+1$).
The regret on iteration $t$ given $Z_{t-1}$ equals
\[
	\E[R_t \mid Z_{t-1}] 
	= \nal + \indi_{\nban > \nal} \frac{\rem}{\amt_{\nal+1}} 
	- \sum_{k=1}^\nban \E \left[ \scc_{k,t} \mid Z_{t-1} \right]
	= \nal + \indi_{\nban > \nal} \frac{\rem}{\amt_{\nal+1}} 
	- \sum_{k=1}^\nban \min\left( 1,\ \frac{\alloc_{k,t}}{\amt_k} \right).
\]
%where, to remind the reader, $\rem$ is the amount of resource allocated to arm $\nal + 1$ in the optimal allocation, and 
%$\mo(\cdot) = \min(1, \cdot)$.
%For any event $A$, let $\indi_A$ be an indicator for $A$.
The next lemma bounds $\E[R_t \mid Z_{t-1}]$, and decomposes it %into
                                %different parts 
in terms of $A_t$, $B_t$ and $C_t$.
\begin{lemma} \label{lem:general}	
	Let $t \in T$. 
	It holds that
	\begin{align}
	\E[\regret_t \mid Z_{t-1}] \le 
	&~~~~\sum_{k \in A_t} \left( 1 - \min\left( \frac{M_{k,t}}{\amt_k},1 \right)\right) \label{eq:gen-l1}\\
	&+ \sum_{k \in A_t} \frac{\add_{k,t}}{\lbf_{k,t-1}} 
	+ \indi_{B_t \ne \emptyset} \frac{\add_t'}{\lbf_{k'_t,t-1}} \label{eq:gen-l2} \\
	&+ \indi_{B_t \cup C_t \ne \emptyset}
	\begin{cases}
	\min(\lbf_{k'_t,t-1}, \alloc_{k'_t,t}) (1/\nu_{\nal+1}-1/\nu_{k'_t}) & |A_t| = \nal \\
	\min(\lbf_{k'_t,t-1}, \alloc_{k'_t,t}) (1/\nu_{\nal}-1/\nu_{k'_t}) & |A_t| < \nal
	\end{cases}. \label{eq:gen-l3}
	\end{align}
\end{lemma}
The proof proceeds by matching between the resource allocated by the optimal allocation, and those of the algorithm.
The amount on line~\eqref{eq:gen-l1} relates to the difference between the reward in the optimal allocation obtained by the first $|A_t|$ arms, and the reward in the algorithm obtained by the members of $A_t$.
The amount on line~\eqref{eq:gen-l2} relates to possibly allocating $\sum_{k \in A_t} \add_{k,t} + \add'_t$
resource to the wrong arms.
%the regret obtained by the fact that some resource given to the arms in $A_t \cup B_t$ could be better utilized.
%More specifically, it relates to an amount of resource of $\sum_{k \in A_t} \add_{k,t} + \add'_t$. This sum can be divided into two parts: 
%the first, $\sum_{k \in A_t} \add_{k,t}$, equals the additional resource allocated to the arms in $A_t$ on top of their lower bounds, namely, 
%$\sum_{k \in A_t} \add_{k,t} = \sum_{k \in A_t} (\alloc_{k,t} - \lbf_{k,t-1})_+$.
%The second part, $\add'_t$, relates to the resource allocated to $k'_t$ if it resides in $B_t$, and if the coin flip tossed in the algorithm decides that all remaining resource will be allocated for it.
Line~\eqref{eq:gen-l3} stands for the regret incurred from allocating $\min(\lbf_{k'_t,t-1}, \alloc_{k'_t,t})$
resources to arm $k'_t$, instead of either to arm $\nal$ or $\nal + 1$.
%
%The idea behind its proof is as follows.
%If $\nal_t \ge \min(\nban, \nal + 1)$, then $|A_t| = \min(\nban, \nal + 1)$, and trivially
%\[
%	\E[R_t \mid Z_{t-1}] \le \sum_{k \in A_t} \para{1 - \mo\para{\alloc_{k,t}/\nu_k}}.
%\]
%Assume therefore that $\nal_t < \min(\nban, \nal + 1)$. It holds that $B_t \cup C_t \ne \emptyset$.
%The first part of the regret,
%$\sum_{k \in A_t} \para{1 - \mo\para{M_{k,t}/\nu_k}}$,
%stands for the difference between the reward obtained by allocating $\alloc_{k,t} = \amt_k$ for all $1 \le k \le \nal_t$, and the reward obtained by allocating arm $k_i$ with $\alloc_{k_i,t}$, for all $1 \le i \le \nal_t$.
%The second part, $\sum_{k \in A_t} \frac{\add_{k,t}}{\lbf_{k,t-1}} + \frac{\add_t'}{\lbf_{k'_t,t-1}}$ stands for
%an amount of $\sum_{k \in A_t} \add_{k,t} + \add_t'$ resource that could be better utilized.
%The last part stands for allocating $\min(\lbf_{k'_t,t-1}, \alloc_{k'_t,t})$ resource to arm $k'_t$ instead of being granted either to arm $\nal$ or to $\nal + 1$.
%
We use Lemma~\ref{lem:general} to bound the total regret on the $n$
iterations by plugging it the second term from the right of
\eqref{eq:term1}, and then changing the order of summation,
\begin{align}
\E R^{(n)}
&= \sum_{t=1}^n \E R_t
= \sum_{t \in T} \E R_t + \sum_{t \notin T} \E R_t
= \sum_{t\in T} \E [\E[ R_t \mid Z_{t-1}]] + \sum_{t \notin T} \E R_t \label{eq:term1}\\
%&= \sum_{t=1}^n \sum_{k \in A_t} \E \para{1 - \mo\para{M_{k,t}/\nu_k}}
%+ \sum_{t=1}^n \sum_{k \in A_t} \E \frac{\add_{k,t}}{\lbf_{k,t-1}} 
%+ \sum_{t=1}^n \indi_{B_t \ne \emptyset} \E \frac{\add_t'}{\lbf_{k'_t,t-1}} \nonumber\\
%&\qquad + \sum_{t=1}^n \indi_{B_t \cup C_t \ne \emptyset} \E \left(
%\begin{cases}
%\min(\lbf_{k'_t,t-1}, \alloc_{k'_t,t}) (1/\nu_{\nal+1}-1/\nu_{k'_t}) & |A_t| = \nal \\
%\min(\lbf_{k'_t,t-1}, \alloc_{k'_t,t}) (1/\nu_{\nal}-1/\nu_{k'_t}) & |A_t| < \nal
%\end{cases}
%\right) 
%+ \sum_{t \notin T} \E R_t \nonumber\\
&= \sum_{k=1}^\nban \sum_{t \colon k \in A_t} \E \left[ 1 - \min\left(\frac{\alloc_{k,t}}{\nu_k}, 1 \right)\right] \label{eq:reg1} \\
&\qquad + \sum_{k=1}^\nban \E \left[\sum_{t \colon k \in A_t} \frac{\add_{k,t}}{\lbf_{k,t-1}} 
+ \sum_{t \colon k \in B_t}^n  \frac{\add_t'}{\lbf_{k,t-1}} \right] \label{eq:reg2}\\
&\qquad + \sum_{k=1}^\nban \E\left[ \sum_{t \colon k \in B_t \cup C_t}
\begin{cases}
\min(\lbf_{k,t-1}, \alloc_{k,t}) (1/\amt_{\nal+1}-1/\amt_{k}) & |A_t| = \nal \\
\min(\lbf_{k,t-1}, \alloc_{k,t}) (1/\amt_{\nal}-1/\amt_{k}) & |A_t| < \nal
\end{cases} \right] \label{eq:reg3} \\
&\qquad + (n-\left\vert T  \right\vert) (\nal + 1). \label{eq:reg4}
\end{align}
In other words, we decompose the regret into four parts,
appearing on lines \eqref{eq:reg1}, \eqref{eq:reg2}, \eqref{eq:reg3} and \eqref{eq:reg4},
each bounded below by a separate lemma.

%Before proceeding to bound the first parts of the regret, we present some auxiliary lemmas.
%We would like to bound the convergence rate of the deterministic lower bound. 
We start with bounding the first two parts, which relate to the
deterministic bound.  Define the \emph{error} of arm $k$ on iteration
$t$ by $\err_{k,t} = \frac{\amt_k - \lbf_{k,t}}{\amt_k}$. We would
like to bound the convergence rate of $\err_{k,t}$ to $0$.
%, or equivalently, $\frac{\lbf_{k,t}}{\amt_k} = 1 - \err_{k,t}$.
%Given any $\epsilon > 0$, we would like to calculate the expected number of iterations that pass before the error $\err_{k,t}$ gets below $\epsilon$.
Since not on every iteration $t$ there are sufficient resources to possibly improve this bound,
every iteration will be counted as $h_{k,t} = \frac{(\alloc_{k,t} - \lbf_{k,t-1})_+}{\add_{k,t}}$ instead of $1$.
Note that $0 \le h_{k,t} \le 1$, and $h_{k,t} = 1$ whenever $k$ is of case A.
%
%However, in some iterations the deterministic bound cannot improve at all.
%This happens in every iteration $t$ for which the allocated amount $\alloc_{k,t}$ is not higher than the lower bound $\lbf_{k,t-1}$.
%This happens when there are no sufficient resource for this arm.
%It can also happen that $\alloc_{k,t} = \lbf_{k,t-1} + \frac{1}{2} \add_{k,t}$, and the optimal case happens when there are sufficient resource and then $\alloc_{k,t} = \lbf_{k,t-1} + \add_{k,t}$.
%The deterministic lower bound can improve on iteration $t$ up to $\lbf_{k,t} = \alloc_{k,t}$.
%Therefore, the higher the difference $\alloc_{k,t} - \lbf_{k,t-1}$ is,
%the higher $\lbf_{k,t} - \lbf_{k,t-1}$ , and the higher the lower bound can improve.

%Define $h_{k,t} = \frac{(\alloc_{k,t} - \lbf_{k,t-1})_+}{\add_{k,t}}$,
%as the ratio between the amount allocated on top of the lower bound,
%and the value it would have got to if there were sufficient resource.
%Every iterations is going to be counted as $h_{k,t}$ instead as $1$,
%when considering the rate of convergence of the deterministic lower bound.
%For instance, in this context, we say that $\sum_{t=t_1+1}^{t_2} h_{k,t}$
%iterations are passed between $t_1$ and $t_2$, instead of $t_2 - t_1$.
%It always holds that $0 \le h_{k,t} \le 1$.

%We will bound the amount of iteration that it takes to the error $\err_{k,t}$ to drop below some $\err > 0$,
%by dividing them into two parts. First, the amount of iterations it takes for the error to drop below some
%constant, denoted as $p$, as stated in Lemma~\ref{lem:start}.
%And then we estimate the number of iterations it takes for the error to drop from $p$ to $\err$, as stated in Lemma~\ref{lem:err-small}.
%This lemma requires that $\mulc(1-p) > 2$, therefore, we define $p = \frac{\mulc-2}{2 \mulc}$.

Define $\rvt_{k,0}$ the lowest value of $t$ for which $\lbf_{k,t} > 0$,
and let $p = \frac{\mulc - 2}{2 \mulc}$.
We start by bounding the number of iterations (weighted by $h_{k,t}$)
that pass from $\rvt_{k,0}$ until the error $\err_{k,t}$ is at most $p$
(equivalently, up to the point that $\lbf_{k,t} \ge (1 - p) \amt_k$).
This number is bounded by $\log \frac{(1-p)\amt_k}{\lbf_{k,\rvt_{k,0}}}$,
which implies that the $\lbf_{k,t}$ grows exponentially fast in the beginning.
Indeed, it grows whenever $\scc_{k,t} = 0$ and this happens with constant probability
in the beginning. Whenever it does, it grows roughly by $\add_{k,t}$,
which is proportional to $\lbf_{k,t}$ in the beginning.
The proof uses a potential function which considers the current values
of $\saf_{k,t}$ and $\lbf_{k,t}$, and bounds the expected number of iterations
up to the desired point.
%
\begin{lemma} \label{lem:start}
	Fix $1 \le k \le \nban$.
	Fix $\gamma \le (1 - p) \amt_k$.
	Let $\rvt$ be the first iteration $t$ that $\lbf_{k,t} \ge \gamma$. Then
	\(
	\E \left[ \sum_{\rvt_{k,0} < t \le \rvt} h_{k,t} \middle\vert \rvt_{k,0},\ \lbf_{k,\rvt_{k,0}} \right]
	\le C \left(\log \frac{\gamma}{\lbf_{k,\rvt_{k,0}}} \right)_+,
	\)
	where $C > 0$ is some universal constant, depending only on $\mulc$.
\end{lemma}
%
Next, for any $0 < \eta < p$, 
we bound the expected number of rounds it takes for the error $\err_{k,t}$
to decrease from $p$ to $\eta$ by around $\frac{1}{\eta}$.
Define by $\rvt_{k,1}$ the first iteration $t$ such that $\err_{k,t} \le p$.
%
\begin{lemma} \label{lem:err-small}
	Fix an integer $k$, $1 \le k \le \nban$.
	Fix some number $0 < \eta < 1$.
	Let $\rvt$ be the first iteration $t$ such that $\err_t \le \eta$.
	Then, there exists a constant $C > 0$ depending only on $\mulc$, such that
	\(
	\E \left[ \sum_{t=\rvt_{k,1}+1}^{\rvt} h_{k,t}
	\middle\vert \rvt_{k,1},\, \saf_{k,\rvt_{k,1}} \right]
	\le C \left( \exp\left( \frac{2 \saf_{k,\rvt_{k,1}}}{\mulc \amt_k (1-p)} \right) + \frac{1}{\eta} \right).
	\)
\end{lemma}
%
This is proved inductively, using a potential function that considers
the current values of $\err_{k,t}$ and $\saf_{k,t}$.  
Intuitively, after $s$ rounds the expected error is around
$\err_{k,t} = \Theta\left(\frac{1}{s}\right)$, and $\add_{k,t}$ is
around $\err_{k,t} / 2$, which implies, by an inductive argument that
the expected error is $\Theta\left(\frac{1}{s+1}\right)$ after $s+1$
rounds.  However, when $\saf_{k,t-1}$ is large, $\add_{k,t}$ is small.
Since $\lbf_{k,t} - \lbf_{k,t-1} \le \add_{k,t}$, a large value of
$\saf_{k,t-1}$ implies that the deterministic lower bound cannot improve
much.  Indeed, the bound of Lemma~\ref{lem:err-small} depends on
$\saf_{k, \rvt_{k,1}}$, which is bounded in the next theorem.
%\yd{next lemma can be removed from outline}
%
\begin{lemma} \label{lem:k-sqr}
	Fix some arm $0 \le k \le \nban$.
	Then, for some constant $C > 0$, 
	\(
	\E\left[ \exp\left( \frac{2 \saf_{k,\rvt_{k,1}}}{\mulc \amt_k (1-p)} \right) \right] \le C,
	\)

\end{lemma}
%
%Next, we are ready to bound the first two parts of the regret, which appear in lines~\eqref{eq:reg1} and \eqref{eq:reg2}. Start with 
%bounding $\eqref{eq:reg1}$, which, for a fixed arm $k$,
%bounds the expected number of failures it performs over the iterations when it resides in $A_t$.
Next, we bound the first part of the regret, appearing on
\eqref{eq:reg1}.
%
\begin{lemma} \label{lem:At} There exists a constant 
$C > 0$,
  depending only on $\mulc$, such that for every arm 
  $k$:
	\(
	\E \left[ \sum_{t \in T \colon k \in A_t} \left(1 -
            \min\left(1, \alloc_{k,t} / \amt_k\right) \right) \right]
        \le C(\log n + \log \nban).
	\)
	%Furthermore, if $k > \nal + 1$, then this expected value is bounded by $c_1(\log \frac{\amt_k}{\amt_k - \amt_{\nal + 1}} + \log \nban)$.
\end{lemma}
%
Recall that whenever $k \in A_t$, it holds that $h_{k,t} = 1$.
First, Lemma~\ref{lem:start} states that it takes $O(\log \nban)$ iterations (weighted by $h_{k,t}$) on expectation
until the error is at most $p$, and the regret from these iterations is $O(\log \nban)$.
Next, we utilize Lemma~\ref{lem:err-small} to bound the regret on the iterations where $\err_{k,t} \le p$.
This lemma, together with Lemma~\ref{lem:k-sqr}, imply that for any $\eta > 0$,
there are on average at most $\frac{C}{\eta}$ iterations (for some constant $C$) from the point that $\err_{k,t} \le p$ to the point that
it equals $\eta$, which means that $C n$ iterations pass before $\err_{k,t} \le \frac{1}{n}$.
Therefore there pass roughly $C$ iterations when the error is between $\frac{1}{n}$ and $\frac{1}{n+1}$.
If we sum the errors $\err_{k,t}$ over all iterations $t \colon k \in A_t$,
we get something similar to a harmonic sum, which is bounded by $C \log n$.
Additionally, whenever $k \in A_t$, $\alloc_{k,t} \ge \lbf_{k,t-1}$,
therefore $1 - \min\left(1, \frac{\alloc_{k,t}}{\amt_k}\right) \le \err_{k,t-1}$, therefore the required sum is at most $C \log n$.
Next, bound the second part of the regret, which appears in line~\eqref{eq:reg2}.

\begin{lemma} \label{lem:add-bound}
	There exists some constant $C > 0$, depending only on $\mulc$,
        such that for every arm $k$: 
	\(
	\E\left[ \sum_{t \in T \colon k \in A_t} \frac{\add_{k,t}}{\lbf_{k,t-1}} 
	+ \sum_{t \in T \colon k \in B_t} \frac{r'_t}{\lbf_{k,t-1}} \right]
	\le C(\log n + \log \nban).
	\)
	%Furthermore, if $k > \nal + 1$, then this value is bounded by $c_2(\log \frac{\amt_k}{\amt_k - \amt_{\nal + 1}} + \log \nban)$.
\end{lemma}

For simplicity, we bound only the sum over iterations $k \in A_t$, dividing into sums
of $\err_{k,t-1} > p$ and $\err_{k,t-1} \le p$.
For the first sum, note that $\frac{\add_{k,t}}{\lbf_{k,t-1}} \le 1$,
and there are only $O(\log \nban)$ iterations in this sum (Lemma~\ref{lem:start})
that contribute together a regret of $O(\log \nban)$.
For the second sum,
we roughly bound $\saf_{k,t} \le \mulc \amt_k \log t$, by induction:
\[
\saf_{k,t}
\le \saf_{k,t} + \add_{k,t}
\le \saf_{k,t-1} + \mulc \amt_k \exp\left( -\frac{\saf_{k,t-1}}{\mulc \amt_k} \right)
\le \mulc \amt_k \log t + \mulc \amt_k \frac{1}{t}
\lesssim \mulc \amt_k \log (t+1).
\]
This implies that approximately
$
\sum_{k \in A_t \colon \lbf_{k,t-1}\ge (1-p)\amt_k} \add_{k,t}
\le \saf_{k,n}
\lesssim \mulc \amt_k \log(n+1)
$,
and dividing each term by $\lbf_{k,t-1} \ge (1-p) \amt_k$
we get a bound of $O(\log n)$.
The case that $k \in B_t$ is slightly more complicated,
and uses the fact that with probability $1/2$, $\lbf_{k,t-1} + \add'_t$
resources are allocated.
Finally, we bound the amount in line~\eqref{eq:reg3}.
%
\begin{lemma} \label{lem:slow} There exists some constant $C > 0$,
  depending only on $\mulc$, such that for every arm $k$:
	\[
	\E\left[ \sum_{t \in T \colon k \in B_t \cup C_t}
	\begin{cases}
	\min(\lbf_{k,t-1}, \alloc_{k,t}) (1/\nu_{\nal+1}-1/\nu_{k}) & |A_t| = \nal \\
	\min(\lbf_{k,t-1}, \alloc_{k,t}) (1/\nu_{\nal}-1/\nu_{k}) & |A_t| < \nal
	\end{cases} \right]
	\le \begin{cases}
	C \frac{\amt_k}{\amt_k - \amt_{\nal + 1}} \log n & k > \nal + 1 \\
	C \frac{\amt_k}{\amt_k - \amt_{\nal}} \log n & k = \nal + 1 \\
	0 & k < \nal + 1
	\end{cases}.
	\]
\end{lemma}
%
The proof of this lemma resembles the proof for UCB by \cite{UCB}.
For $k = 0$ this bounded amount is trivially zero.  For
$k > \nal + 1$, whenever the probabilistic lower bound is sufficiently
tight, arm $k$ will not be in $B_t \cup C_t$ anymore, since it has to
be one of the $\nal + 1$ arms with the lowest lower bound
$\lb_{k,t-1}$ in order to be in
$B_t \cup C_t$.  Whenever $k \in B_t \cup C_t$, the probabilistic
bound improves with constant probability 
(partially due to the randomness of allocating case B),
therefore Azuma bound ensures that
after a sufficient amount of time
$\lbs_{k,t}$ is sufficiently tight indeed. The case that
$k = \nal + 1$ is analyzed similarly.
This concludes the proof sketch of Theorem~\ref{thm:multi-arm}.
A full proof appears in \appref{sec:proof:thm:multi-arm}.

==> multi-outline_part_3.tex <==
This concludes the proof sketch of Theorem~\ref{thm:multi-arm}. Due to lack of space we defer all details to the supplementary material. 
A full proof appears in \appref{sec:proof:thm:multi-arm}.


==> proof-outline-long.tex <==
\section{Proof outline of Theorem~\ref{thm:multi-arm}} \label{sec:pr-outline}
We sketch an outline of the proof, which contains the
main idea and a summary of their proofs.  The proofs of the lemmas,
together with a list of all definitions appears in the appendix. The
algorithm receives an constant which for the purpose of analysis we
assume $c>2$.
%  This
% section contains many technical definitions, which are, for
% themselves, not very interesting, yet they are essential for
% understanding the proof and all lemmas are based on then.  Since the
% algorithm does not know the number of iterations in advance, it is
% impossible to make adjustments to the algorithm that rely on this
% information.  This complicates the proof and requires us to analyze
% the behavior of the algorithm for any state it gets to, which results
% in a highly technical proof.

% We bound the expected regret of the algorithm after $n$ rounds if it
% interacts with the fixed arms $\amt_1, \dots, \amt_\nban$.  The
% algorithm gets as an input a parameter $\mulc$, which is used for
% calculating the value of $\add_{k,t}$.  It is conseders as a constant
% ,and indeed, it can get any constant value higher than $2$, to the
% choice of the user.

The algorithm maintains a lower bound $\lb_{k,t}$ for any arm $1 \le k \le \nban$ and iteration $1 \le t \le n$.
Most of the proof relates only to iterations $t$ such that for any arm $k$, this lower bound is positive and less than $\amt_k$.
Let $T$ be the set of these iterations, namely, 
\[  T = \{ t \colon 1 \le t \le n,\ 0 < \lb_{k,t} \le \amt_k \text{ for all } 1 \le k \le \nban \}. \]
For iterations $t \notin T$, we use the trivial bound $R_t \le \nal +
1$. Below in \lemref{lem:notin-T} we show that the number of such
iterations is constant in $n$.

% the regret $R_t$ is bounded trivially as if no reward is gained from these iterations, namely, we bound $R_t \le \nal + 1$.
% Later on this outline, we state a lemma that bounds the expected number of iterations not in $T$.

We start by describing how the regret is bounded in ``good
iterations'' when $t \in T$.  The optimal allocation that knows the
parameters $\amt_1, \dots, \amt_k$, allocates the first $\nal$ arms
with the amount they require, and the next arm gets the remaining of
the resources (this happens in case there is no sufficient resource
for all arms.  There are $\nal + 1$ arms which are allocated with a
non-negative amount of resource.  The regret in an iteration $t \in T$
is calculated by comparing the reward obtained by the ``optimal''
allocation, with the reward obtained by at most $\nal + 1$ arms in the
algorithm.  For this purpose, three sets of arms, $A_t$, $B_t$ and
$C_t$, will be defined, and only the reward of the arms in these sets
is going to be considered for the calculation of the regret.
Optimally, the set $A_t$ would contain the $\nal$ arms that get the
highest priority by the algorithm on iteration $t$, where the arm with
the next priority is going to be located either in $B_t$ or $C_t$: one
of these two sets is going to be a singleton which contains only this
arm, and the other is going to be empty.  In reality, however, $A_t$
is not necessarily going to contain exactly $\nal$ arms. It might be
the case that $A_t$ contains $\nal + 1$ arms, and when it happens
$B_t$ and $C_t$ are both empty.  Additionally, $A_t$ can be of size
less than $\nal$.  It holds that $A_t$, $B_t$ and $C_t$ are subsets of
the sets of arms labeled by $A$, $B$ and $C$ by the algorithm on
iteration $t$, respectively.

Next, we give a formal definitions of the sets $A_t$, $B_t$ and $C_t$.
Fix some iteration $1 \le t \le n$.
Let $k_{1,t}, \dots, k_{\nban,t}$ be an ordering of the arms such that arm $k_i$ is dealt with in iteration $i$ in the loop over the arms in line~\ref{algl:k-loop} which defines their priority in getting the resources.
From the definition of the algorithm it holds that this ordering sorts the bandits in an increasing order of their maximum lower bound $\lb_{k,t} = \max(\lbf_{k,t}, \lbs_{k,t})$, namely $\lb_{k_{1,t},t-1} \le \lb_{k_{2,t},t-1} \le \cdots \le \lb_{k_{\nban,t},t-1}$.

Let $\nal_t$ be the number of iterations passed in the loop in line~\ref{algl:k-loop} before encountering an arm $k$ for which there are no sufficient resources, namely, the amount of resources left is less than $\lbf_{k,t-1} + \add_{k,t}$. 
Formally, $\nal_t$ is the highest value of $i$ such that for all 
$1 \le j \le i$, $\alloc_{k_{j,t}, t} = \lbf_{k_{j,t},t-1} + \add_{k_{j,t},t}$.
Let $A_t$ be the set that contains the first $\nal+1$ arms encountered in that loop before the first time that there was an arm which did not have sufficient resources, or, in other words, $A_t$ contains the first $\min(\nal_t, \nal + 1)$ arms encountered in the loop. Formally,
\[
A_t = \{ k_{1,t}, k_{2,t}, \dots, k_{\min(\nal_t, \nal+1),t} \}.
\]

If $A_t$ contains less than $\nal + 1$ arms, and does not contain all the arms,
let $k'_t$ be the next arm encountered in the loop after the arms which resides in $A_t$.
Formally, $k'_t = k_{|A_t|+1,t}$, and it is defined only if $|A_t| < \min(\nban, \nal + 1)$.
It holds that the remaining resources for $k'_t$ on iteration $t$ are less than $\lbf_{k,t-1} + \add_{k,t}$,
otherwise it would have been placed in $A_t$.
The arm $k'_t$ is either placed in $B_t$ or in $C_t$: if the remaining resources for $k'_t$ surpass the lower bound $\lbf_{k,t-1}$, then $B_t = \{ k'_t \}$ and $C_t = \emptyset$ (the actual amount of resource given to $k'_t$ is not necessarily higher than $\lbf_{k,t-1}$. This is defined depending on the random coin flip performed by the algorithm).
If the amount of resources remaining is not higher than the lower bound, we set $C_t = \{k'_t \}$ and $B_t = \emptyset$.
If $k'_t$ is not defined at all, which happens whenever $A_t$ is sufficiently large, then $B_t = C_t = \emptyset$.
Here is the formal definition of $B_t$ and $C_t$:
\begin{align*}
B_t &= \begin{cases}
\{k'_t \} & |A_t| < \min(\nal + 1,\nban) \ \BR{AND}\  1 - \sum_{k \in A_t} \alloc_{k,t} > \lbf_{k'_t,t-1} \\
\emptyset & \BR{otherwise}
\end{cases}, \\
C_t &= \begin{cases}
\{k'_t \} & |A_t| < \min(\nal + 1,\nban) \ \BR{AND}\  1 - \sum_{k \in A_t} \alloc_{k,t} \le \lbf_{k'_t,t-1} \\
\emptyset & \BR{otherwise}
\end{cases}.
\end{align*}
If $B_t \ne \emptyset$, define by $\add'_t$ the amount of resources left for $k'_t$ minus its lower bound $\lbf_{k'_t,t-1}$.
From the definition of $B_t$, this value is guaranteed to be positive.
If $B_t = \emptyset$ then this value has no meaning and is defined to be $0$.
Formally,
\[
\add'_t = \begin{cases}
1 - \sum_{k \in A_t} \alloc_k - \lbf_{k'_t,t-1} & B_t \ne \emptyset \\
0 & B_t = \emptyset
\end{cases}.
\]

Define by $Z_t$ the random variable that contains everything the algorithm has seen up to and just before the point it gets to see the success statuses of the arms on iteration $t+1$. It contains all the success statuses $\scc_{k,i}$ for any arm $1 \le k \le \nban$ and any iteration $1 \le i \le t$, in addition to all the randomness of the algorithm up to and including iteration $t + 1$.
Particularly, the amounts allocated to the arms on iteration $t+1$, namely, $\alloc_{1,t+1}, \dots, \alloc_{\nban, t+1}$, are deterministically defined given $Z_t$.
The expected regret in iteration $t$ given $Z_{t-1}$ therefore equals the expected reward of the optimal algorithm, 
minus the expected reward of Algorithm~\eqref{alg:multi-arm}, which equals
\[
\E[R_t \mid Z_{t-1}] 
= \nal + \indi_{\nban > \nal} \frac{\rem}{\amt_{\nal+1}} 
- \sum_{k=1}^\nban \E \scc_{k,t}
= \nal + \indi_{\nban > \nal} \frac{\rem}{\amt_{\nal+1}} 
- \sum_{k=1}^\nban \mo\left( \frac{\alloc_{k,t}}{\amt_k} \right),
\]
where, to remind the reader, $\rem$ is the amount of resource allocated to arm $\nal + 1$ in the optimal allocation, and 
$\mo(\cdot) = \min(1, \cdot)$.
For any event $A$, let $\indi_A$ be an indicator for $A$.
The next lemma bounds $\E[R_t \mid Z_{t-1}]$, and decomposes it into different parts in terms of $A_t$, $B_t$ and $C_t$.

\begin{lemma} \label{lem:general}	
	Let $t \in T$. 
	It holds that
	\begin{align}
	\E[\regret_t \mid Z_{t-1}] \le 
	&\sum_{k \in A_t} \para{1 - \mo\para{M_{k,t}/\nu_k}} \label{eq:gen-l1}\\
	&+ \sum_{k \in A_t} \frac{\add_{k,t}}{\lbf_{k,t-1}} 
	+ \indi_{B_t \ne \emptyset} \frac{\add_t'}{\lbf_{k'_t,t-1}} \label{eq:gen-l2} \\
	&+ \indi_{B_t \cup C_t \ne \emptyset}
	\begin{cases}
	\min(\lbf_{k'_t,t-1}, \alloc_{k'_t,t}) (1/\nu_{\nal+1}-1/\nu_{k'_t}) & |A_t| = \nal \\
	\min(\lbf_{k'_t,t-1}, \alloc_{k'_t,t}) (1/\nu_{\nal}-1/\nu_{k'_t}) & |A_t| < \nal
	\end{cases}. \label{eq:gen-l3}
	\end{align}
\end{lemma}

The proof matches between the resource allocated by the optimal allocation, 
and those of the algorithm.
The amount on line~\eqref{eq:gen-l1} relates to the difference between the reward in the optimal allocation obtained by the first $|A_t|$ arms, and the reward in the algorithm obtained by the members of $A_t$.
The amount on line~\eqref{eq:gen-l2} relates to the regret obtained by the fact that some resource given to the arms in $A_t \cup B_t$ could be better utilized. More specifically, it relates to an amount of resources of $\sum_{k \in A_t} \add_{k,t} + \add'_t$. This sum can be divided into two parts: 
the first, $\sum_{k \in A_t} \add_{k,t}$, equals the additional resource allocated to the arms in $A_t$ on top of their lower bounds, namely, 
$\sum_{k \in A_t} \add_{k,t} = \sum_{k \in A_t} (\alloc_{k,t} - \lbf_{k,t-1})_+$.
The second part, $\add'_t$, relates to the resource allocated to $k'_t$ if it resides in $B_t$, and if the coin flip tossed in the algorithm decides that all remaining resources will be allocated for it.
Line~\eqref{eq:gen-l3} stands for the regret incurred from allocating an amount of $\min(\lbf_{k'_t,t-1}, \alloc_{k'_t,t})$ resources to arm $k'_t$, instead of being allocated either to arm $\nal$ or to $\nal + 1$.



%The idea behind its proof is as follows.
%If $\nal_t \ge \min(\nban, \nal + 1)$, then $|A_t| = \min(\nban, \nal + 1)$, and trivially
%\[
%	\E[R_t \mid Z_{t-1}] \le \sum_{k \in A_t} \para{1 - \mo\para{\alloc_{k,t}/\nu_k}}.
%\]
%Assume therefore that $\nal_t < \min(\nban, \nal + 1)$. It holds that $B_t \cup C_t \ne \emptyset$.
%The first part of the regret,
%$\sum_{k \in A_t} \para{1 - \mo\para{M_{k,t}/\nu_k}}$,
%stands for the difference between the reward obtained by allocating $\alloc_{k,t} = \amt_k$ for all $1 \le k \le \nal_t$, and the reward obtained by allocating arm $k_i$ with $\alloc_{k_i,t}$, for all $1 \le i \le \nal_t$.
%The second part, $\sum_{k \in A_t} \frac{\add_{k,t}}{\lbf_{k,t-1}} + \frac{\add_t'}{\lbf_{k'_t,t-1}}$ stands for
%an amount of $\sum_{k \in A_t} \add_{k,t} + \add_t'$ resources that could be better utilized.
%The last part stands for allocating $\min(\lbf_{k'_t,t-1}, \alloc_{k'_t,t})$ resources to arm $k'_t$ instead of being granted either to arm $\nal$ or to $\nal + 1$.

Based on Lemma~\ref{lem:general}, we can bound the total regret on the $n$ iterations by
\begin{align}
\E R^{(n)}
&= \sum_{t=1}^n \E R_t
= \sum_{t \in T} \E R_t + \sum_{t \notin T} \E R_t
= \sum_{t\in T} \E [\E[ R_t \mid Z_{t-1}]] \nonumber + \sum_{t \notin T} \E R_t \\
&= \sum_{t=1}^n \sum_{k \in A_t} \E \para{1 - \mo\para{M_{k,t}/\nu_k}}
+ \sum_{t=1}^n \sum_{k \in A_t} \E \frac{\add_{k,t}}{\lbf_{k,t-1}} 
+ \sum_{t=1}^n \indi_{B_t \ne \emptyset} \E \frac{\add_t'}{\lbf_{k'_t,t-1}} \nonumber\\
&\qquad + \sum_{t=1}^n \indi_{B_t \cup C_t \ne \emptyset} \E \left(
\begin{cases}
\min(\lbf_{k'_t,t-1}, \alloc_{k'_t,t}) (1/\nu_{\nal+1}-1/\nu_{k'_t}) & |A_t| = \nal \\
\min(\lbf_{k'_t,t-1}, \alloc_{k'_t,t}) (1/\nu_{\nal}-1/\nu_{k'_t}) & |A_t| < \nal
\end{cases}
\right) 
+ \sum_{t \notin T} \E R_t \nonumber\\
&= \sum_{k=1}^\nban \sum_{t \colon k \in A_t} \E \para{1 - \mo\para{\alloc_{k,t}/\nu_k}} \label{eq:reg1} \\
&\qquad + \sum_{k=1}^\nban \E \left[\sum_{t \colon k \in A_t} \frac{\add_{k,t}}{\lbf_{k,t-1}} 
+ \sum_{t \colon k \in B_t}^n  \frac{\add_t'}{\lbf_{k,t-1}} \right] \label{eq:reg2}\\
&\qquad + \sum_{k=1}^\nban \E\left[ \sum_{t \colon k \in B_t \cup C_t}
\begin{cases}
\min(\lbf_{k,t-1}, \alloc_{k,t}) (1/\amt_{\nal+1}-1/\amt_{k}) & |A_t| = \nal \\
\min(\lbf_{k,t-1}, \alloc_{k,t}) (1/\amt_{\nal}-1/\amt_{k}) & |A_t| < \nal
\end{cases} \right] \label{eq:reg3} \\
&\qquad + \left| \{1, \dots, n \} \setminus T  \right| (\nal + 1). \label{eq:reg4}
\end{align}

The regret is decomposed into four parts,
appearing on lines \eqref{eq:reg1}, \eqref{eq:reg2}, \eqref{eq:reg3} and \eqref{eq:reg4},
each will be bounded by a separate lemma.


Before proceeding to bound the first parts of the regret, we present some auxiliary lemmas.
We would like to bound the convergence rate of the deterministic lower bound. 
Define the \emph{error} of arm $k$ on iteration $t$ by $\err_{k,t} = \frac{\amt_k - \lbf_{k,t}}{\amt_k}$, or equivalently, $\frac{\lbf_{k,t}}{\amt_k} = 1 - \err_{k,t}$.
Given any $\epsilon > 0$, we would like to calculate the expected number of iterations that pass before the error $\err_{k,t}$ gets below $\epsilon$.
However, in some iterations the deterministic bound cannot improve at all.
This happens in every iteration $t$ for which the allocated amount $\alloc_{k,t}$ is not higher than the lower bound $\lbf_{k,t-1}$.
This happens when there are no sufficient resources for this arm.
It can also happen that $\alloc_{k,t} = \lbf_{k,t-1} + \frac{1}{2} \add_{k,t}$, and the optimal case happens when there are sufficient resources and then $\alloc_{k,t} = \lbf_{k,t-1} + \add_{k,t}$.
The deterministic lower bound can improve on iteration $t$ up to $\lbf_{k,t} = \alloc_{k,t}$.
Therefore, the higher the difference $\alloc_{k,t} - \lbf_{k,t-1}$ is,
the higher $\lbf_{k,t} - \lbf_{k,t-1}$ , and the higher the lower bound can improve.

Define $h_{k,t} = \frac{(\alloc_{k,t} - \lbf_{k,t-1})_+}{\add_{k,t}}$,
as the ratio between the amount allocated on top of the lower bound,
and the value it would have got to if there were sufficient resources.
Every iterations is going to be counted as $h_{k,t}$ instead as $1$,
when considering the rate of convergence of the deterministic lower bound.
For instance, in this context, we say that $\sum_{t=t_1+1}^{t_2} h_{k,t}$
iterations are passed between $t_1$ and $t_2$, instead of $t_2 - t_1$.
It always holds that $0 \le h_{k,t} \le 1$.

We will bound the amount of iteration that it takes to the error $\err_{k,t}$ to drop below some $\err > 0$,
by dividing them into two parts. First, the amount of iterations it takes for the error to drop below some
constant, denoted as $p$, as stated in Lemma~\ref{lem:start}.
And then we estimate the number of iterations it takes for the error to drop from $p$ to $\err$, as stated in Lemma~\ref{lem:err-small}.
This lemma requires that $\mulc(1-p) > 2$, therefore, we define $p = \frac{\mulc-2}{2 \mulc}$.

We start by presenting Lemma~\ref{lem:start}.
For any $\epsilon' \le p$, this lemma bounds the expected number of iterations that
pass from the first iteration $t$ that $\lbf_{k,t} > 0$, up to the point that $\err_{k,t} \le \epsilon'$.
This can be stated equivalently as follows: for every $\gamma \le (1-p) \amt_k$,
the lemma bounds the number of iterations that pass up to the point that $\lbf_{k,t} \ge (1-p) \amt_k$.
Formally, for any arm $1 \le k \le \nban$, define $\rvt_{k,0}$ as the lowest value of $t$ for which $\lbf_{k,t} > 0$.

\begin{lemma} \label{lem:start}
	Fix $1 \le k \le \nban$.
	Fix $\gamma \le (1 - p) \amt_k$.
	Let $\rvt$ be the first iteration $t$ that $\lbf_{k,t} \ge \gamma$. Then
	\[
	\E \left[ \sum_{\rvt_{k,0} < t \le \rvt} h_{k,t} \middle\vert \rvt_{k,0},\ \lbf_{k,\rvt_{k,0}} \right]
	\le C \left(\log \frac{\gamma}{\lbf_{k,\rvt_{k,0}}} \right)_+,
	\]
	where $C > 0$ is some universal constant, depending only on $\mulc$.
\end{lemma}

On other words, the lemma states that it takes an order of $\log \frac{\gamma}{\lbf_{k,\rvt_{k,0}}}$
iterations for the deterministic lower bound to change from $\lbf_{k,\rvt_{k,0}}$ to $\gamma$,
which means that it grows exponentially fast.
Assume for simplicity that in every iteration there are sufficient resources to an arm $k$, so that 
$\alloc_{k,t} = \lbf_{k,t-1} + \add_{k,t}$, and $h_{k,t} = 1$.
For most iterations $t$, the lower bound 
grows by an amount proportional to its size,
with constant probability.
To state it differently, $\lbf_{k,t} - \lbf_{k,t-1}$
is at least some constant times $\lbf_{k,t-1}$, with constant probability.

We start by arguing why the lower bound grows with constant probability.
Note that it grows whenever the arm fails, namely, $\lbf_{k,t} > \lbf_{k,t-1}$ whenever $\scc_{k,t} = 0$.
This happens with probability
\[
1 - \min\left( 1, \frac{\alloc_{k,t}}{\amt_k} \right)
\ge 1 - \frac{\lbf_{k,t-1} + \add_{k,t}}{\amt_k}
= \err_{k,t-1} - \frac{\add_{k,t}}{\amt_k}
\ge p - \frac{\add_{k,t}}{\amt_k},
\]
where the last inequality holds since we are considering only iterations where the 
error is at most $p$.
Therefore, if  $\frac{\add_{k,t}}{\amt_k}$ is sufficiently smaller than $p$, then the lower bound grows with high probability.
For reminder, it holds that
\[ \add_{k,t} = \lbf_{k,t-1} \mulc \exp \left( -\frac{\saf_{k,t}}{\mulc \amt_k} \right). \]
It holds that $\saf_{k,t} = \sum_{i \le t \colon \lbf_{k,t} > 0} (\alloc_{k,t} - \lbf_{k,t-1})_+$,
the sum of the amount of allocated resource on top of the lower bound, constantly increases. 
Therefore, whenever the lower bound does not change, $\add_{k,t}$ decreases.
After a constant number of iterations that the lower bound does not change, $\add_{k,t}$ will be sufficiently small, and the probability of failure of arm $k$ would be sufficiently large.

Next, we explain why whenever the lower bound increases,
the amount by which it increases is proportional to the lower bound.
The amount of increase, $\lbf_{k,t} - \lbf_{k,t-1}$, equals $\add_{k,t}$,
since we assumed for simplicity that there is lack of resources.
We expect $\frac{\saf_{k,t}}{\lbf_{k,t-1}}$ to be at most some constant, with high probability.
Although $\saf_{k,t}$ increases every iteration, $\lbf_{k,t-1}$ keeps the pace.
Therefore, the formula for $\add_{k,t}$ equals a constant times $\lbf_{k,t-1}$, and indeed, $\add_{k,t}$ is of the same magnitude as $\lbf_{k,t-1}$.

The actual proof is by induction, using a potential function, which considers both the current lower bound, and the current value of $\add_{k,t}$, and bounds the expected time it takes for the lower bound to be at least $\gamma$.
We could not apply standard concentration bounds to prove this lemma.
Consider the following problem.
If by a chance arm $k$ has very few failures, then $\lbf_{k,t}$ does not increase much,
while $\saf_{k,t}$ does.
This causes $\add_{k,t}$ to be low.
Since the lower bound bound can increase by at most $\add_{k,t}$, it cannot increase greatly.
With non negligible probability, $\add_{k,t}$ can get considerably low, and it is impossible to bound this event as unlikely to happen. It is required to consider also cases where $\add_{k,t}$ is very small, and this is done by the potential function.

%
%The lemma says that in order for the deterministic lower bound to get from $\lbf_{k,\rvt_{k,0}}$ to $\gamma$, $\log \frac{\gamma}{\lbf_{k,\rvt_{k,0}}}$ iterations are passed, which means that $\lbf_{k,t}$ grows exponentially fast.
%We will show that for most iterations $\rvt_{k,0} < t \le \rvt$,
%it holds that $\lbf_{k,t} - \lbf_{k,t-1} = \Omega(1) \lbf_{k,t-1}$ with constant probability, which means that the deterministic bound is indeed expected to grow exponentially fast.
%Assume for simplicity that $h_{k,t}$ always equals 1.
%The difference $\lbf_{k,t} - \lbf_{k,t-1}$ equals either $\add_{k,t}$ or zero, depending on $\scc_{k,t}$.
%It holds that
%\begin{align} 
%	\Pr[\lbf_{k,t} - \lbf_{k,t-1} = \add_{k,t}]
%	= \Pr[\scc_{k,t} = 0]
%	= 1 - \mo\left( \frac{\alloc_{k,t}}{\amt_k} \right) 
%	\ge 1 - \frac{\lbf_{k,t-1} + \add_{k,t}}{\amt_k} \\
%	\ge p - \frac{\add_{k,t}}{\amt_k}
%	\ge p - \mulc \exp\left( - \frac{\saf_{k,t-1}}{\mulc \lbf_{k,t-1}} \right).
%\end{align}
%Assuming that $\saf_{k,t-1}$ is sufficiently large, it follows that $\lbf_{k,t} - \lbf_{k,t-1} = \add_{k,t}$
%with constant probability. If $\saf_{k,t-1}$ is too small, then we can wait a constant number of iterations until it grows to the desired value.
%
%We will explain why $\add_{k,t}$ is expected to be in the same order of $\lbf_{k,t-1}$, and this will conclude that $\lbf_{k,t}$
%grows exponentially fast.
%In every iteration $\rvt_{k,0} < t \le \rvt$, it holds that $\saf_{k,t} - \saf_{k,t-1} = (\alloc_{k,t} - \lbf_{k,t-1})_+ = \add_{k,t}$ (under the assumption $h_{k,t} = 1$).
%On the other hand, $\lbf_{k,t} - \lbf_{k,t-1}$ equals $\add_{k,t}$ with a constant probability and 0 otherwise.
%Therefore, $\lbf_{k,t-1} = \sum_{i=\rvt_{k,0}}^{t-1} (\lbf_{k,i} - \lbf_{k,i-1})$ is expected to be a constant times 
%$\saf_{k,t-1} = \sum_{i=\rvt_{k,0}}^{t-1} (\saf_{k,i} - \saf_{k,i-1})$.
%This implies that 
%$\add_{k,t} 
%= \lbf_{k,t-1} \mulc \exp\left(- \frac{\saf_{k,t-1}}{\mulc \lbf_{k,t-1}} \right)
%=\lbf_{k,t-1} \Theta(1)$, as required.

Next, for any $0 < \eta < p$, we estimate the number of rounds it takes for the lower bound error, $\err_{k,t}$, to get below $\eta$, from the point it equals $p$.
Define by $\rvt_{k,1}$ the first iteration $t$ such that $\err_{k,t} \le p$.

\begin{lemma} \label{lem:err-small}
	Fix an integer $k$, $1 \le k \le \nban$.
	Fix some number $0 < \eta < 1$.
	Let $\rvt$ be the first iteration $t$ such that $\err_t \le \eta$.
	Then,
	\[
	\E \left[ \sum_{t=\rvt_{k,1}+1}^{\rvt} h_{k,t}
	\middle\vert \rvt_{k,1},\, \saf_{\rvt_{k,1}} \right]
	\le C \left( \exp\left( \frac{2 \saf_{\rvt_{k,1}}}{\mulc \amt_k (1-p)} \right) + \frac{1}{\eta} \right),
	\]
	for some constant $C > 0$ depending only on $\mulc$.
\end{lemma}

This is proved inductively, using a potential function, that bounds the time it takes for the error
to get below $\eta$, given the current values of $\err_{k,t}$ and $\saf_{k,t}$.
We give some intuition about the proof.
Fix an iteration $t$, and assume for simplicity that $h_{k,t} = 1$, namely, $\alloc_{k,t} = \lbf_{k,t-1} + \add_{k,t}$.
It holds that $\lbf_{k,t} - \lbf_{k,t-1} = \add_{k,t}$ whenever the arm fails (whenever $\scc_{k,t} = 0$). 
This happens with probability 
\[
\max\left(0, 1 - \frac{\alloc_{k,t}}{\amt_k} \right) 
= \max\left(0, 1 - \frac{\lbf_{k,t-1}+ \add_{k,t}}{\amt_k} \right)
= \max\left(0, \err_{k,t-1} - \frac{\add_{k,t}}{\amt_k} \right).
\]
Therefore, on expectation, the difference between $\lbf_{k,t}$ and $\lbf_{k,t-1}$ equals 
$\max\left(0, \err_{k,t} - \frac{\add_{k,t}}{\amt_k} \right) \add_{k,t}$.
The optimal value for $\add_{k,t}$ is obtained when $\frac{\add_{k,t}}{\amt_k} = \frac{1}{2} \err_{k,t}$.
Indeed, $\add_{k,t}$ would usually be of the same magnitude as $\frac{1}{2} \amt_k \err_{k,t}$.
However, it can be significantly lower or higher than that quantity, and the proof characterizes the 
behavior of the algorithm in each of these cases.
Another detail taken care of is the fact that a change in the lower bound can greatly change the value of $\add_{k,t}$.

As can be seen, the bound in Lemma~\ref{lem:err-small} depends on $\saf_{\rvt_{k,1}}$, the sum of differences between the allocations and their corresponding lower bounds, 
up to the first time that the error $\err_{k,t}$ is below $p$.
Indeed, if this value is too large, then the values of $\add_{k,t}$ are going to be very small, and the deterministic lower bound will not be able to increase fast: recall that the lower bound can increase by at most $\add_{k,t}$.
Therefore, we have to bound the value of $\saf_{\rvt_{k,1}}$, as done in the next lemma.

\begin{lemma} \label{lem:k-sqr}
	Fix some arm $0 \le k \le \nban$.
	Then,
	\[
	\E\left[ \exp\left( \frac{2 \saf_{\rvt_{k,1}}}{\mulc \amt_k (1-p)} \right) \right] \le C,
	\]
	for some constant $C > 0$.
\end{lemma}

Next, we are ready to bound the first two parts of the regret, which appear in lines~\eqref{eq:reg1} and \eqref{eq:reg2}. Start with 
bounding $\eqref{eq:reg1}$, which, for a fixed arm $k$,
bounds the expected number of failures it performs over the iterations when it resides in $A_t$.

\begin{lemma} \label{lem:At}
	There exists a constant $c_1 > 0$, depending only on $\mulc$, such that for every arm $k$, $1 \le k \le \nban$:
	\[
	\E \left[ \sum_{t \in T \colon k \in A_t} (1 - \mo(\alloc_{k,t} / \amt_k)) \right] \le c_1(\log n + \log \nban).
	\]
	%Furthermore, if $k > \nal + 1$, then this expected value is bounded by $c_1(\log \frac{\amt_k}{\amt_k - \amt_{\nal + 1}} + \log \nban)$.
\end{lemma}

In order to prove this theorem, note that Lemma~\ref{lem:start} implies that it takes $O(\log \nban)$ 
rounds before the error $\err_{k,t}$ is below $p$,
and lemmas \ref{lem:err-small} and \ref{lem:k-sqr}
imply that it takes $O(\frac{1}{\eta})$ iterations on average from that point,
up to the point that $\err_{k,t} \le \eta$, for all $\eta > 0$.
Summing these contributions, it takes $O(\log \nban + \frac{1}{\eta})$
iterations before the error gets below $\eta$.
This fact is utilized in the proof: if $t \in A_t$,
then the amount allocated is at least the lower bound $\lbf_{k,t-1}$.
If the error $\err_{k,t-1}$ is low, then the allocated amount is not considerably lower than $\amt_k$,
therefore, the failure probability is going to be low.

Additionally, note that whenever $k \in A_t$, it holds that $h_{k,t} = \frac{(\alloc_{k,t} - \lbf_{k,t-1})_+}{\add_{k,t}} = 1$, namely, the iteration is counted as $1$ in the lemmas regarding the convergence of $\lbf_{k,t}$ towards $\amt_k$.
Therefore, every time that $k \in A_t$ contributes to improving the deterministic bound.

Next, bound the second part, which appears in line~\eqref{eq:reg2}.

\begin{lemma} \label{lem:add-bound}
	There exists some constant $c_2 > 0$, depending only on $\mulc$, such that for every arm $k$, $1 \le k \le \nban$:
	\[
	\E\left[ \sum_{t \in T \colon k \in A_t} \frac{\add_{k,t}}{\lbf_{k,t-1}} 
	+ \sum_{t \in T \colon k \in B_t} \frac{r'_t}{\lbf_{k,t-1}} \right]
	\le c_2(\log n + \log \nban).
	\]
	%Furthermore, if $k > \nal + 1$, then this value is bounded by $c_2(\log \frac{\amt_k}{\amt_k - \amt_{\nal + 1}} + \log \nban)$.
\end{lemma}

First, the lower bound quickly passes $(1-p)\amt_k$,
as proved in Lemma~\ref{lem:start}.
Summing the values of $\add_{k,t}$ and $\add'_t$ only over all iterations for which $\lbf_{k,t-1} \ge (1-p) \amt_k$, we get that
\begin{equation} \label{eq:int-add}
\E\left[ \sum_{\substack{t \in T \colon k \in A_t \\ \lbf_{k,t-1} \ge (1-p)\amt_k}} \add_{k,t} 
+ \sum_{\substack{t \in T \colon k \in B_t \\ \lbf_{k,t-1} \ge (1-p)\amt_k}} \add'_t \right] 
\le 2 \sum_{t=1}^n (\alloc_{k,t} - \lbf_{k,t-1})_+
= 2 \sum_{t=1}^n h_{k,t} \add_{k,t}
= O(\amt_k \log n).
\end{equation}
The first inequality follows from the following reasons. Firstly, whenever $k \in A_t$, it holds that $\alloc_{k,t} - \lbf_{k,t-1} = \add_{k,t}$. Secondly, whenever $k\in B_t$, it holds that with probability $1/2$, $\alloc_{k,t} - \lbf_{k,t-1} = \add'_t$, and with probability $1/2$ it equals zero, therefore, on expectation, it equals $2 (\alloc_{k,t} - \lbf_{k,t-1})$.
The second equality follows from definition of $h_{k,t}$.
The last equality follows from the fact that the sequence of values $\add_{k,1}, \add_{k,2}, \cdots$
is constructed such that it behaves similarly to $\frac{\amt_k \mulc}{1}, \frac{\amt_k \mulc}{2}, \dots$.
Dividing each summand in \eqref{eq:int-add} by $\lbf_{k,t-1} \ge (1-p)\amt_k$, we get a bound of $O(\log n)$. 

Next, we bound the amount in line~\eqref{eq:reg3}.

\begin{lemma} \label{lem:slow}
	There exists some constant $c_2 > 0$, depending only on $\mulc$, such that for every arm $k$, $1 \le k \le \nban$:
	\[
	\E\left[ \sum_{t \in T \colon k \in B_t \cup C_t}
	\begin{cases}
	\min(\lbf_{k,t-1}, \alloc_{k,t}) (1/\nu_{\nal+1}-1/\nu_{k}) & |A_t| = \nal \\
	\min(\lbf_{k,t-1}, \alloc_{k,t}) (1/\nu_{\nal}-1/\nu_{k}) & |A_t| < \nal
	\end{cases} \right]
	\le \begin{cases}
	c_3 \frac{\amt_k}{\amt_k - \amt_{\nal + 1}} \log n & k > \nal + 1 \\
	c_3 \frac{\amt_k}{\amt_k - \amt_{\nal}} \log n & k = \nal + 1 \\
	0 & k < \nal + 1
	\end{cases}.
	\]
\end{lemma}

This bound is proved by estimating the convergence rate of the
probabilistic lower bound $\lbs_{k,t}$ to $\amt_k$.
Note that for any $k < \nal + 1$ the bound is trivially correct.
Assume that $k > \nal + 1$, and the case that $k = \nal + 1$ is dealt in a similar fashion.
For any arm $k$, we expect that for any iteration $1 \le j \le n$,
$\sum_{t \le j \colon k \in B_t \cup C_t} \min(\lbf_{k,t-1}, \alloc_{k,t})$
will be at most twice the value of
$\sas_{k,j}$ (the sum of allocations $1 \le t \le j$ for which the amount allocated is at most the lower bound).
Therefore, whenever the sum that we wish to bound is $\Omega(\log n)$, then
so $\sas_{k,t}$.
Using concentration bounds for martingales
we can show that if $\sas_{k,j} = \Omega(\log n)$,
then the probabilistic lower bound is going to be sufficiently tight.
The tightness of the lower bound implies that arm $k$ is not going to be prioritized high enough to be a part of 
$B_t \cup C_t$ anymore: it has to be prioritized among top $\nal +1$ arms in order to be a part of these sets,
while its priority under the optimal policy is lower than $\nal + 1$, since we assumed that $k < \nal + 1$.
Therefore, the sum will stop growing from that point onwards.

Now, we describe why the sum $\sum_{t \le j \colon k \in B_t \cup C_t} \min(\lbf_{k,t-1}, \alloc_{k,t})$
is expected to be at most twice the size of $\sas_{k,j}$.
We will explain why on every iteration $t$, the difference $\sas_{k,t} - \sas_{k,t-1}$
is on expectation between half the size to the size of $\min(\lbf_{k,t-1}, \alloc_{k,t})$, and this will imply the result,
by summing over $t \le j$.
If an arm $k$ is in $C_t$, then the amount of resources allocated to it is at most the lower bound, 
therefore  $\sas_{k,t}$ is increased by $\alloc_{k,t} = \min(\lbf_{k,t-1}, \alloc_{k,t})$.
If $k \in B_t$, then the amount allocated is at least the lower bound, therefore
$\min(\lbf_{k,t-1}, \alloc_{k,t}) = \lbf_{k,t-1}$.
With probability half the amount allocated equals $\lbf_{k,t-1}$.
In that case, $\sas_{k,t}$ is greater than $\sas_{k,t-1}$ by $\lbf_{k,t-1} = \min(\lbf_{k,t-1}, \alloc_{k,t})$,
as required. With probability half the amount allocated is higher than $\lbf_{k,t-1}$, and $\sas_{k,t} = \sas_{k,t-1}$.

%To sketch the proof, note that if $k \le \nal$, then this bound trivially equals zero.
%Assume that $k > \nal + 1$.
%In every iteration $t$ that $k \in C_t$, it holds that $\alloc_{k,t} \le \lbf_{k,t-1}$, therefore 
%$\sas_{k,t} = \sas_{k,t-1} + \alloc_{k,t} = \sas_{k,t-1} + \min(\lbf_{k,t-1}, \alloc_{k,t})$.
%In every iteration $t$ that $k \in B_t$, it holds that with probability $1/2$, 
%$\alloc_{k,t} = \lbf_{k,t-1}$, and therefore $\sas_{k,t} = \sas_{k,t-1} + \alloc_{k,t} = \sas_{k,t-1} + \min(\lbf_{k,t-1}, \alloc_{k,t})$.
%On the other hand, with probability $1/2$ it holds that $\alloc_{k,t} > \lbf_{k,t-1}$, and in this case $\sas_{k,t} = \sas_{k,t-1}$.
%Therefore, regardless of whether $k\in B_t$ or $k \in C_t$, $\sas_{k,j}$ is expected to be around at least half the value of $\sum_{t \le j \colon k \in B_t \cup C_t,\ t\in T} \min(\lbf_{k,t-1}, \alloc_{k,t})$.
%
%If for some $1 \le j \le n$ it holds that
%\[ \sum_{t \le j \colon k \in B_t \cup C_t,\ t\in T} \min(\lbf_{k,t-1}, \alloc_{k,t}) = \Omega\left( \frac{\amt_k}{\amt_k - \amt_{\nal+1}} (1/\amt_{\nal+1} - 1/\amt_k)^{-1} \right) \]
%it holds that with high probability, 
%\[ \sas_{k, j} 
%= \Omega\left( \frac{\amt_k}{\amt_k - \amt_{\nal+1}} (1/\amt_{\nal+1} - 1/\amt_k)^{-1} \right) 
%=\Omega\left( \frac{1/\amt_{\nal+1}}{(1/\amt_{\nal+1} - 1/\amt_k)^2} \right). \]
%Concentration bounds show that whenever this happens, with high probability $\lbs_{k,j} > \amt_{\nal+1}$.
%If this happens, it does not hold that $k \in B_j \cup C_j$, as will soon be explained.
%Therefore, 
%\[ \sum_{t \in T \colon k \in B_t \cup C_t} \min(\lbf_{k,t-1}, \alloc_{k,t}) (1/\amt_{\nal+1} - 1/\amt_k) \] 
%is expected to be in the order of $\frac{\amt_k}{\amt_k - \amt_{\nal+1}}$ as required.
%
%Next, we show why whenever $\lbs_{k,t} > \amt_{\nal+1}$, it holds that $k \notin B_t \cup C_t$.
%Assuming that $t \in T$, for every arm $i \le \nal + 1$ it holds that 
%$\lb_{i,t-1} \le \amt_i \le \amt_{\nal + 1} < \lbs_{k,t}$.
%This implies that there are at least $\nal + 1$ arms which are going to be iterated before $k$ in the loop in line \cmt{REF}.
%From the definitions of $B_t$ and $C_t$ this implies that $k \notin B_t \cup C_t$.
%To complete the proof we have to bound the corresponding sum that relates to arm $\nal +1$ instead of $\nal$, and consider the case that $k = \nal+1$. This is proved similarly.


Lastly, we bound the amount on line~\eqref{eq:reg4}, 
by bounding the number of iterations not in $T$, namely, the iterations for which there exists an arm $k$
for which either $\lb_{k,t-1} > \amt_k$, or $\lb_{k,t-1} = 0$.
This quantity is bounded by $O\left(\max\left(\log \frac{1}{\amt_1}, 1\right)\right)$.

\begin{lemma} \label{lem:notin-T}
	There exists a constant $c_4 > 0$, depending only on $\mulc$,
	such that the expected number of iterations $t$, $1 \le t \le n$,
	for which $t \notin T$, is bonded by
	$c_4 \max\left(\log \frac{1}{\amt_1}, 1\right)$.
\end{lemma}

The proof consists of two part.
The first one, proved in Lemma~\ref{lem:first-bd},
bounds the number of iterations for which there exists an arm $k$
such that the lower bound, $\lb_{k,t-1}$, is zero.
As described in the proof, every arm has an initialization phase,
where in every iteration the amount of resources given to it is halved,
until the arm fails in its task, and a value of $\scc_{k,t} = 0$ is returned.
Whenever this happens, a deterministic positive lower bound is set,
and it will never get back to zero.
Since the amount of resource given to an arm in the initialization process is halved on every iteration,
it is not going to take long before the arm fails for the first time.

The second part of the proof of this lemma consists of bounding the number of iterations $t$
such that there exists $k$ for which the lower bound,
$\lb_{k,t}$ is greater than $\amt_k$,
and is proved in Lemma~\ref{lem:bad-slow-bd}.
This is done by proving that for any arm $1 \le k \le \nban$ and iteration $1 \le t \le n$,
the probability that $\lb_{k,t} > \amt_k$ is at most $\frac{1}{t^2 \nban}$.
A sum over $t$ and $k$ results in a bound of $O(1)$ on the expected number of "bad" iterations.
Note that $\lb_{k,t} > \amt_k$ if and only if $\lbs_{k,t} > \amt_k$.
This is true since $\lb_{k,t} = \max\left(\lbf_{k,t}, \lbs_{k,t}\right)$,
and the deterministic bound, $\lbf_{k,t}$, is always less than $\amt_k$.
The estimation of the probability that $\lbs_{k,t} > \amt_k$
is calculated using a martingale concentration bound.



%Here is a sketch of the proof.
%The expected number of iterations $t$ for which there exists $k$ such that $\lb_{k,t} = 0$ is bounded by $\max\left(\log \frac{1}{\amt_1}, 1\right) + O(1)$, as proved in Lemma~\ref{lem:first-bd}.
%In short, we prove that for all $t \ge \log \frac{1}{\amt_1} + 2$,
%it holds that with probability at least $1/2$,
%all arms $k$ for which $\lb_{k,t-1} = 0$ satisfy $\lb_{k,t} = 0$.
%Indeed, for all $t \ge \log \frac{1}{\amt_1} + 2$, and for all $k$, it holds that
%\[
%	\Pr[\lb_{k,t} = 0 | \lb_{k,t-1} = 0]
%	= \Pr[\scc_{k,t} = 1 | \lb_{k,t-1} = 0]
%	\le \frac{\alloc_{k,t}}{\amt_k}
%	\le \frac{\amt_1}{2 \nban \amt_k}
%	\le \frac{1}{2\nban},
%\]
%where $\alloc_{k,t} = \frac{1}{\nban 2^{t-1}}$,
%and a union bound over $k$ derives the result.
%
%The expected number of iterations $t$ for which there exists $k$ such that $\lb_{k,t} > \amt_k$ 
%is bounded by $O(1)$ as proved in Lemma~\ref{lem:bad-slow-bd}.
%Since $\lb_{k,t} = \max(\lbf_{k,t}, \lbs_{k,t})$, and it always holds that $\lbf_{k,t} \le \amt_k$, it is sufficient to bound the number of iterations that $\lbs_{k,t} > \amt_k$.
%This is done by using a martingale inequality,
%and proving that for every $1 \le t \le n$ and $1 \le k \le \nban$, 
%it holds that $\Pr[\lbs_{k,t} > \amt_k] = O\left( \frac{1}{t^2 \nban} \right)$.
%A union bound over $k = 1, \dots, \nban$ and $t=1,\dots, n$ derives the result.


==> proofsa.tex <==
\yd{Proof moved to the exclusive section, which, in turn, will move to the appendix.}

%
%\subsection{Proof of Theorem~\ref{thm:om}}\label{sec:proof:thm:om}
%Fix an arm $1 \le k \le \nban$.
%Let $n'$ be the number of times that arm $k$ is invoked throughout the $n$ iterations of the algorithm,
%and let $t_1 < \cdots < t_{n'}$ be these iterations.
%We start by proving item~\ref{itm:th-om-1}.
%It is sufficient to prove that 
%\begin{equation} \label{eq:omm-0}
%	\E \left[ \sum_{i=1}^{n'} (\alloc_{t_i} - \amt^*) \right] 
%	\le \min\left( c \log n, C \log \frac{1}{\amt_k - \amt^*} + C \right).
%\end{equation}
%
%The guarantee for the one-arm problem, proved in Theorem~\ref{thm:ub-one},
%states that the left hand side of \eqref{eq:omm-0} is bounded by $c \log n$.
%Next, we prove that it is bounded by $C \log \frac{1}{\amt_k - \amt^*}$, whenever $\amt_k > \amt^*$, to complete the proof of \eqref{eq:omm-0}.
%
%Assume therefore that $\amt_k > \amt^*$.
%Next, we show that for all $1 \le i \le n'$,
%\begin{equation} \label{eq:omm-3}
%	\lb_{k,t_i-1} < \amt^*.
%\end{equation}
%Since arm $k$ is invoked by the algorithm on iteration $t_i$, it has the minimal lower bound on this iteration, namely,
%$\lb_{k,t_i-1} = \min_{1\le s \le \nban} \lb_{s,t_i-1}$.
%Let $s$ be the arm which satisfies $\amt_s = \amt^*$.
%It holds that $\lb_{k,t_i - 1} \le \lb_{s,t_i - 1} < \amt_s = \amt^*$, which completes the proof of \eqref{eq:omm-3}.
%
%Let $n_1 = \min \para{n', \left\lceil \frac{2 \mulc}{\amt - \amt^*}\right\rceil - 1}$.
%We will split the left hand side of \eqref{eq:omm-0} to two sums, one from $1$ to $n_1$,
%and the other from $n_1+1$ to $n'$.
%The first sum is bounded by
%\begin{align}
%	\sum_{i=1}^{n_1} (\alloc_{t_i} - \amt^*)
%	&= \sum_{i=1}^{n_1} \left(\lb_{k,t_i - 1} + \frac{\mulc}{i} - \amt^* \right) \nonumber\\
%	&\le \sum_{i=1}^{n_1} \frac{\mulc}{i} \label{eq:omm2} \\
%	& \le \mulc \para{ \log n_1 + 1} \nonumber \\
%	& \le \mulc \para{ \log \frac{2 \mulc}{\amt - \amt^*} + 1} \nonumber.
%\end{align}
%where \eqref{eq:omm2} follows from \eqref{eq:omm-3}.
%
%Proceed with bounding the sum from $n_1+1$ to $n'$.
%If $n' = n_1$ it trivially equals zero, therefore assume that $n' > n_1$.
%For any $n_1 < i \le n'$ it holds that
%\begin{equation} \label{eq:omm4}
%	\alloc_{t_i}
%	= \lb_{k,t_i-1} + \frac{\mulc}{i}
%	\le \amt^* + \frac{\mulc}{n_1+1}
%	\le \amt^* + \frac{\amt_k - \amt^*}{2}.
%\end{equation}
%where the second step follows from \eqref{eq:omm-3}.
%
%Let $i_1 < \cdots < i_m$ denote all values of $n_1 < i \le n'$, for which $\alloc_{t_i} > \amt^*$.
%It holds that
%\begin{align}
%	\sum_{i=n_1+1}^{n'} (\alloc_{t_i} - \amt^*)
%	&\le \sum_{j=1}^{m} (\alloc_{t_{i_j}} - \amt^*) \nonumber\\
%	&\le \sum_{j=1}^{m} \frac{\amt_k - \amt^*}{2} \label{eq:omm5} \\
%	&= m \frac{\amt_k - \amt^*}{2} \nonumber,
%\end{align}
%where \eqref{eq:omm5} follows from \eqref{eq:omm4}.
%We will show that $\E m \le \frac{2}{\amt_k - \amt^*}$,
%thereby, completing the proof of \eqref{eq:omm-0}.
%
%First, note that for any $j < m$ it holds that
%the arm succeeds on iteration $t_{i_j}$, namely, 
%$\scc_{t_{i_j}} = 1$.
%Otherwise, it would hold that
%\[
%\lb_{k, t_{i_{j+1}}}
%\ge \lb_{k, t_{i_{j}}}
%= \alloc_{k, t_{i_{j}}}
%> \amt_k,
%\]
%where the first and second steps follow from the definition of the algorithm,
%and the last step follows from the definition of $j_1, \dots, j_m$.
%This contradicts \eqref{eq:omm-3}, and proves that $\scc_{t_{i_j}} = 1$ 
%for all $j < m$ as required.
%
%For any $1 \le j \le m$, \eqref{eq:omm4} implies that
%$\amt_k - \alloc_{t_{i_j}} \ge \frac{\amt_k - \amt^*}{2}$.
%The definition of the problem implies that the probability that the arm fails on iteration $t_{i_j}$, and $\scc_{t_{i_j}} = 0$,
%is at least $\amt_k - \alloc_{t_{i_j}} \ge \frac{\amt_k - \amt^*}{2}$.
%Viewing $m$ as a random variable, this implies that for any integer $j > 0$, 
%\[
%\Pr[m \ge j + 1 \mid m \ge j]
%\le \Pr\left[\alloc_{t_{i_j}} = 1 \mid m \ge j \right]
%\le 1 - \frac{\amt_k - \amt^*}{2}.
%\]
%Therefore, $m$ can be bounded by a geometric random variable with parameter $\frac{\amt_k - \amt^*}{2}$,
%which implies that $\E m \le \frac{2}{\amt_k - \amt^*}$ as required. This completes the proof of \eqref{eq:omm-0},
%and item~\ref{itm:th-om-1} of the theorem follows.
%
%Next, we prove the second part of the theorem.
%It is sufficient to prove that
%\begin{equation} \label{eq:omm2-m}
%	\E \left[ \sum_{i=1}^{n'} (1 - \scc_{t_i}) \right] 
%	\le \min\left( \frac{\mulc}{\mulc-1} \log n, C \log \frac{1}{\amt_k - \amt^*} + C \right).
%\end{equation}
%Using Theorem~\ref{thm:ub-one} for the one-arm problem,
%it holds that 
%\[
%\E \left[ \sum_{i=1}^{n'} (1 - \scc_{t_i}) \right] 
%\le \frac{\mulc}{\mulc-1} \log n.
%\]
%Next, we will bound this quantity by $C \log \frac{1}{\amt_k - \amt^*} + C$
%assuming that $\amt_k > \amt^*$, and it suffices to complete the proof.
%Inequality~\eqref{eq:omm-3} implies that it suffices to bound the number of failures of arm $k$
%before the first iteration $t$ when $\lb_{k,t} \ge \amt^*$.
%This implies that the following lemma suffices to complete the proof.
%
%\begin{lemma}
%	Fix some $0 < a < \amt \le 1$.
%	Assume that the one armed algorithm, Algorithm~\ref{alg:one-arm}, runs and interacts with an arm with parameter $\amt$,
%	and gets an input parameter $\mulc > 1$.
%	Let $\alloc_t$, $\scc_t$ and $\lb_t$ be defined as in the algorithm for all $t = 1,2,\cdots$.
%	Let $\rvt$ be the first iteration $t$ such that $\lb_t > a$.
%	Then,
%	\[ \E\left[ \sum_{t=1}^{\rvt} (1 - \scc_t) \right] \le C\log \frac{1}{\amt - a} + C, \]
%	where $C > 0$ is some parameter which depends only on $\mulc$.
%\end{lemma}
%
%\begin{proof}
%	We will prove that for any iteration $t \ge 1$, and any value $0 \le \lb_{t-1} < \amt$,
%	\begin{equation} \label{eq:om-main}
%		\E \left[ \sum_{i=t}^{\rvt} (1 - \scc_i) \middle\vert t, \lb_{t-1} \right]
%		\le \phi(\amt - \lb_{t-1}, t),
%	\end{equation}
%	where
%	\[
%	\phi(\err,t) = c_1 \left( \log \frac{2 \err}{\amt - a} \right)_+ + c_2 (\err t - \alpha)_+,
%	\]
%	where the function $(\cdot)_+$ denotes $\max(0, \cdot)$, and 
%	\begin{align*}
%		\gamma_1 &= \frac{2 \mulc^2}{\mulc - 1} \\
%		\alpha &= \gamma_1 + 1 \\
%		\gamma_2 &= \alpha + \mulc \\
%		c_2 &= \frac{2}{\mulc-1} \\
%		c_1 &= \frac{2 c_2 + 1}{\log \frac{1}{1 - \mulc / \gamma_2}}.
%	\end{align*}
%	Whenever $\amt - \lb_{t-1} < \amt - a$, the left hand side of inequality~\eqref{eq:om-main} is trivially zero,
%	and the right hand side is always nonnegative, therefore \eqref{eq:om-main} holds.
%	Therefore, for the next of the proof we assume thats $\amt - \lb_{t-1} < \amt - a$.
%	
%	Fix some values of $t$ and $\lb_{t-1}$.
%	Denote $\err = \amt - \lb_{t-1}$. Denote $t_0 = t_1 = t$.
%	Denote by $\err_0$ the value $\amt - \lb_t$ gets if $\scc_t = 0$, namely, $\err_0 = (\err - \frac{\mulc}{t})_+$.
%	Similarly, let $\err_1$ be the value of $\amt - \lb_t$ if $\scc_t = 1$, namely, $\err_1 = \err$.
%	Let $p$ be the probability that $\scc_t$ equals $0$, given $\lb_{t-1}$.
%	In order to prove \eqref{eq:om-main}, it is sufficient to prove the following inductive inequality:
%	\begin{equation} \label{eq:om-rec}
%		\phi(\err, t) \ge p \left( \phi(\err_0, t_0) + 1 \right) + (1-p) \phi(\err_1, t_1) .
%	\end{equation}
%	
%	The proof of \eqref{eq:om-rec} will be divided into cases.
%	First, it assumes that $\err_ 0 \ge \frac{\amt - a}{2}$,
%	and proves for each of the following three cases:
%	$t \err < \gamma_1$, $\gamma_1 \le t \err \le \gamma_2$,
%	and $t \err > \gamma_2$.
%	Lastly, it proves for the case that $\err_ 0 \ge \frac{\amt - a}{2}$.
%	
%	Start by assuming that $\err_ 0 \ge \frac{\amt - a}{2}$.
%	It holds that, $\log \frac{2 \err_0}{\amt - a} \ge 0$, therefore
%	\begin{equation} \label{eq:om-e0-good}
%		\left( \log \frac{2 \err_0}{\amt - a} \right)_+
%		= \log \frac{2 \err_0}{\amt - a}.
%	\end{equation}
%	
%	It holds that if $t \err \le \gamma_2$,
%	then 
%	\begin{equation} \label{eq:om-0}
%		c_1 \log \frac{\err}{\err_0} - 1 
%		= c_1 \log \frac{\err}{\err - \mulc/t} - 1 
%		= c_1 \log \frac{1}{1 - \mulc/(\err t)} - 1 
%		\ge c_1 \log \frac{1}{1 - \mulc/\gamma_2} - 1 
%		= 2 c_2.
%	\end{equation}
%	
%	If $t \err \ge \gamma_1$, then
%	\begin{equation} \label{eq:om-1}
%		\err_0
%		= \err - \frac{\mulc}{t}
%		= \err \left( 1 - \frac{\mulc}{\err t} \right)
%		\ge \err \left( 1 - \frac{\mulc}{\gamma_1} \right)
%		= \err \left( 1 - \frac{\mulc(\mulc - 1)}{2 \mulc^2} \right)
%		\ge \err / 2.
%	\end{equation}
%	Therefore, if $t \err \ge \gamma_1$ then 
%	\begin{equation} \label{eq:om-2}
%		p = \err - \frac{\mulc}{t} \ge \err / 2.
%	\end{equation}
%	
%	Therefore, if $\gamma_1 \le t \err \le \gamma_2$, then
%	\begin{align}
%		&\phi(\err, t) - p \left( \phi(\err_0, t_0) + 1 \right) - (1-p) \phi(\err_1, t_1) \nonumber\\
%		&= -p + p c_1 \log \frac{\err}{\err_0} + c_2 (\err t - \alpha)_+ 
%		- p c_2(\err_0(t+1) - \alpha)_+ - (1-p) c_2(\err_1(t+1) - \alpha)_+ \label{eq:om-3} \\
%		&\ge -p + p c_1 \log \frac{\err}{\err_0} + c_2 (\err t - \alpha)_+ - c_2(\err(t+1) - \alpha)_+ \nonumber\\
%		&\ge p \left( c_1 \log \frac{\err}{\err_0} - 1 \right) - c_2 \err \nonumber \\
%		&\ge \frac{2p}{c_2} - c_2 \err \label{eq:om-4} \\
%		&\ge 0. \label{eq:om-5} \\
%	\end{align}
%	where \eqref{eq:om-3} follows from \eqref{eq:om-e0-good},
%	\eqref{eq:om-4} follows from \eqref{eq:om-0},
%	and \eqref{eq:om-5} follows from \eqref{eq:om-2}.
%	This concludes the proof of \eqref{eq:om-rec} for the case that $\gamma_1 \le t \err \le \gamma_2$.
%	
%	Next, assume that $t \err > \gamma_2$. Then,
%	\begin{equation} \label{eq:om-6}
%		t \err_0
%		= t \left( \err - \frac{\mulc}{t} \right)
%		= t \err - \mulc.
%	\end{equation}
%	Therefore,
%	\begin{equation} \label{eq:om-7}
%		t \err
%		\ge t \err_0
%		\ge t \err - \mulc
%		\ge \gamma_2 - \mulc
%		= \alpha.
%	\end{equation}
%	Additionally,
%	\begin{equation} \label{eq:om-10}
%		\mulc p - \err
%		= \mulc \left( \err - \frac{\mulc}{t} \right) - \err 
%		= \err \left( \mulc - 1 - \frac{\mulc^2}{\err t} \right)
%		\ge \err \left( \mulc - 1 - \frac{\mulc^2}{\gamma_2} \right)
%		\ge \err \left( \mulc - 1 - \frac{\mulc^2}{\gamma_1} \right)
%		= \frac{\mulc - 1}{2} \err.
%	\end{equation}
%	This concludes that,
%	\begin{align}
%		&\phi(\err, t) - p \left( \phi(\err_0, t_0) + 1 \right) - (1-p) \phi(\err_1, t_1) \nonumber \\
%		&\ge -p + c_2 (\err t - \alpha)_+ - p c_2 (\err_0 (t+1) - \alpha)_+ - (1-p)c_2 (\err_1 (t+1) - \alpha)_+ \nonumber \\
%		&= -p + c_2 \left( \err t - p \err_0 (t+1) - (1-p) \err (t+1) \right)\label{eq:om-8} \\
%		&\ge -p + c_2 \left( p(\err t - \err_0 t) - \err \right) \nonumber \\
%		&= -p + c_2 (\mulc p - \err) \label{eq:om-9} \\
%		&\ge -p + c_2 \frac{\mulc - 1}{2} \err  \label{eq:om-11} \\
%		&= -p + \err \nonumber \\
%		&\ge 0 \nonumber.
%	\end{align}
%	where \eqref{eq:om-8} follows from \eqref{eq:om-7},
%	\eqref{eq:om-9} follows from \eqref{eq:om-6},
%	and \eqref{eq:om-11} follows from \eqref{eq:om-10}.
%	This completes the proof for the case that $\err t > \gamma_2$.
%	
%	Next, assume that $\err t < \gamma_1$.
%	This implies that
%	\begin{equation} \label{eq:om-12}
%		\err (t+1)  
%		= \err t + \err
%		\le \gamma_1 + 1
%		= \alpha.
%	\end{equation}
%	Therefore,
%	\begin{align}
%		&\phi(\err, t) - p \left( \phi(\err_0, t_0) + 1 \right) - (1-p) \phi(\err_1, t_1) \nonumber \\
%		&= p(c_1 \log \frac{\err}{\err_0} - 1) \label{eq:om-13} \\
%		&\ge 2 p c_2 \label{eq:om-14} \\
%		&\ge 0,
%	\end{align}
%	where \eqref{eq:om-13} follows from \eqref{eq:om-12} and \eqref{eq:om-e0-good},
%	and \eqref{eq:om-14} follows from \eqref{eq:om-0}.
%	This completes the proof of \eqref{eq:om-rec} for the case $\err t < \gamma_1$.
%	
%	Lastly, assume that $\err_0 < \frac{\amt-a}{2}$.
%	It holds that
%	\begin{equation*}
%		\frac{c}{\gamma_2}
%		\le \frac{c}{\gamma_1}
%		= \frac{c(c-1)}{2 c^2}
%		\le \frac{1}{2}.
%	\end{equation*}
%	Therefore, 
%	\begin{equation} \label{eq:om-15}
%		c_1
%		\ge \log^{-1} \frac{1}{1-c/\gamma_2}
%		\ge \log^{-1} 2.
%	\end{equation}
%	Additionally, since $\err_0 < \frac{\amt-a}{2}$, 
%	it holds that $t \err < \gamma_1$, otherwise \eqref{eq:om-1} would imply that
%	$\err_0 \ge \frac{\err}{2} \ge \frac{\amt-a}{2}$.
%	Therefore, \eqref{eq:om-12} holds.
%	For conclusion,
%	\begin{align}
%		&\phi(\err, t) - p \left( \phi(\err_0, t_0) + 1 \right) - (1-p) \phi(\err_1, t_1) \nonumber \\
%		&= -p + p c_1 \log \frac{2\err}{\amt - a} \label{eq:om-16} \\
%		&\ge -p + p c_1 \log 2 \nonumber \\
%		&\ge 0 \label{eq:om-17}
%	\end{align}
%	where \eqref{eq:om-16} follows from \eqref{eq:om-12},
%	and \eqref{eq:om-17} follows from \eqref{eq:om-15}.
%	This completes the proof of \eqref{eq:om-rec},
%	and the proof of the theorem follows.
%\end{proof}
%


==> related.tex <==
\paragraph{Related Work:} 
The problem was first suggested by \cite{LCS}.
Their solution was inspired by the \emph{upper confidence interval} (UCB) algorithm of \cite{UCB}
for the stochastic multi armed bandit problem.
The algorithm of \citeauthor{LCS} maintains high probability lower bound estimates on the parameters
$\amt_1, \dots, \amt_\nban$.
On every iteration $t$, the arms are prioritized by these bounds, from the lowest to the highest,
each arm getting an amount of resources which equals its lower bound, until no resource is left.
Using this technique, the best arms get almost all the resource they require,
hence, their probability of success is close to $1$, and their outcomes have a low variance.
This enables the writers to estimate $\amt_k$ with a standard deviation of
$\Theta\left( \frac{1}{t} \right)$ after $t$ allocations.
Yet, the proof requires the constructed lower bound estimates to hold throughout all the $n$ iterations,
which implies that their failure probability has to be low.
This high confidence requirement weakens the tightness of this constructed estimate,
contributing a multiplicative factor of $\log n$ to the regret.
We eliminate this logarithmic factor by replacing the probabilistic lower bounds with deterministic ones,
utilizing the fact that the error is one-sided:
if arm $k$ is allocated with $\alloc$ resources and terminates in failure,
we know that $\amt_k > \alloc$ with probability $1$.

This problem belongs to the class of stochastic partial monitoring problems, first studied by \cite{RAT89}.
These are exploration vs. exploitation problems,
where the user performs actions and obtains a stochastic reward based on them,
and on an additional hidden parameter.
See \cite{LCS} for relevant literature on this topic, including the work by \cite{BM12}.
Another related field is R{\'e}nyi--Ulam games, or, searching with errors.
This is a class of problems aimed at revealing a hidden element by asking questions, while some 
of the answers may be erroneous.
In our settings, the hidden element is $\amt_k$, and granting an arm with an amount 
$\alloc$ of resource can be viewed as asking the question: ``is $\amt_k \ge \alloc_k$?''.
\cite{SEARCH02} has written an extensive survey,
mainly dealing with worst case guarantees under limitations on the errors.
\cite{KAR07}, \cite{JED12} and \cite{WEB13} suggested models with stochastic error.
The model discussed in our paper was generalized by \cite{LCS2}, to enable multiple resource types.
They discuss the relation to stochastic linear bandits (eg. \cite{AYSC11} and \cite{AR13}) and online combinatorial optimization (\cite{KBW15}).


==> stuff.tex <==

\section{generalizations - to be removed}

\begin{itemize}
	\item 
	What happens if the amount of resources available change between days?
	\item
	What if different arms can have a different reward?
	\item
	What if we have one arm and multiple resources, and the amount of required resources, and it requires some fixed amount from every resource.
	\item
	Show that in the one-arm case we can get a constant regret if our arm requires more than 1 amount of money to succeed.
	\item
	In the one arm case: if the optimum is not at allocating all resources, then the lower bound is $\Omega(\sqrt{n})$. Should we also construct an algorithm for that case?
\end{itemize}


